Holistic Network Virtualization and Pervasive Network Intelligence for 6G

In this tutorial paper, we look into the evolution and prospect of network architecture and propose a novel conceptual architecture for the 6th generation (6G) networks. The proposed architecture has two key elements, i.e., holistic network virtualization and pervasive artificial intelligence (AI). The holistic network virtualization consists of network slicing and digital twin, from the aspects of service provision and service demand, respectively, to incorporate service-centric and user-centric networking. The pervasive network intelligence integrates AI into future networks from the perspectives of networking for AI and AI for networking, respectively. Building on holistic network virtualization and pervasive network intelligence, the proposed architecture can facilitate three types of interplay, i.e., the interplay between digital twin and network slicing paradigms, between model-driven and data-driven methods for network management, and between virtualization and AI, to maximize the flexibility, scalability, adaptivity, and intelligence for 6G networks. We also identify challenges and open issues related to the proposed architecture. By providing our vision, we aim to inspire further discussions and developments on the potential architecture of 6G.

==> Bios.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.3in,clip,keepaspectratio]{./Fig/Xuemin Shen}}]{Xuemin (Sherman) Shen} (Fellow, IEEE)  received the Ph.D. degree in electrical engineering from Rutgers University, New Brunswick, NJ, USA, in 1990. He is a University Professor with the Department of Electrical and Computer Engineering, University of Waterloo, Canada. His research focuses on network resource management, wireless network security, Internet of Things, 5G and beyond, and vehicular networks. Dr. Shen is a registered Professional Engineer of Ontario, Canada, an Engineering Institute of Canada Fellow, a Canadian Academy of Engineering Fellow, a Royal Society of Canada Fellow, a Chinese Academy of Engineering Foreign Member, and a Distinguished Lecturer of the IEEE Vehicular Technology Society and Communications Society. 

Dr. Shen received the Canadian Award for Telecommunications Research from the Canadian Society of Information Theory (CSIT) in 2021, the R.A. Fessenden Award in 2019 from IEEE, Canada, Award of Merit from the Federation of Chinese Canadian Professionals (Ontario) in 2019, James Evans Avant Garde Award in 2018 from the IEEE Vehicular Technology Society, Joseph LoCicero Award in 2015 and Education Award in 2017 from the IEEE Communications Society (ComSoc), and Technical Recognition Award from Wireless Communications Technical Committee (2019) and AHSN Technical Committee (2013). He has also received the Excellent Graduate Supervision Award in 2006 from the University of Waterloo and the Premiers Research Excellence Award (PREA) in 2003 from the Province of Ontario, Canada. He served as the Technical Program Committee Chair/Co-Chair for IEEE GLOBECOM’16, IEEE INFOCOM’14, IEEE VTC’10 Fall, IEEE GLOBECOM’07, and the Chair for the IEEE ComSoc Technical Committee on Wireless Communications. Dr. Shen is the President Elect of the IEEE ComSoc. He was the Vice President for Technical\&Educational Activities, Vice President for Publications, Member-at-Large on the Board of Governors, Chair of the Distinguished Lecturer Selection Committee, and Member of IEEE Fellow Selection Committee of the ComSoc. Dr. Shen served as the Editor-in-Chief of the IEEE IoT JOURNAL, IEEE Network, and IET Communications. 

% received the B.Sc. degree in electrical engineering from Dalian Maritime University, Dalian, China, in 1982, and the M.Sc. and Ph.D. degrees in electrical engineering from Rutgers University, Camden, NJ,
% USA, in 1987 and 1990, respectively.

% He is currently a University Professor from the Department of Electrical and Computer Engineering, University of Waterloo, Waterloo, ON, Canada. His research interests include resource management in interconnected wireless/wired networks, wireless network security, social networks, smart grid, and vehicular ad hoc and sensor networks. 

% Dr. Shen was a recipient of the Excellent Graduate Supervision Award in 2006, the Outstanding Performance Award from the University of Waterloo, in 2004, 2007, 2010, and 2014, the Premier’s Research Excellence Award (PREA) from the Province of Ontario, Canada, in 2003, the Distinguished Performance Award from the Faculty of Engineering, University of Waterloo, in 2002 and 2007, and the Joseph LoCicero Award from the IEEE Communications Society. He served as the Technical Program Committee Chair/Co-Chair for the IEEE Global Communications Conference (GLOBECOM) 2016 and IEEE International Conference on Computer Communications, 2014, the IEEE Vehicular Technology Conference (VTC), 2010, and GLOBECOM’07, the Symposia Chair for the IEEE International Conference on Communications (ICC), 2010, the Tutorial Chair for the IEEE VTC’11 Spring and the IEEE ICC’08, the General Co-Chair for International Symposium on Mobile Ad-Hoc Networking and Computing, 2015, International Conference on Communications and Networking in China, 2007, and International ICST Conference on Quality of Service in Heterogeneous Wired/Wireless Networks, 2006, and the Chair for
% the IEEE Communications Society Technical Committee on Wireless Communications, and P2P Communications and Networking. He also serves/served as the Editor-in-Chief for the IEEE INTERNET OF THINGS JOURNAL, the IEEE NETWORK, Peer-to-Peer Networking and Application, and IET Communications, a Founding Area Editor for the IEEE TRANSACTIONS ON WIRELESS COMMUNICATIONS, and an Associate Editor for the IEEE TRANSACTIONS ON VEHICULAR TECHNOLOGY, Computer Networks, and ACM/Wireless Networks. He is a Registered Professional Engineer of ON, Canada, an Engineering Institute of Canada Fellow, a Canadian Academy of Engineering Fellow, a Royal Society of Canada Fellow, and a Distinguished Lecturer of the IEEE Vehicular Technology Society and Communications Society.
%received the  B.Sc.(1982) degree from Dalian Maritime University (China) and the M.Sc. (1987) and Ph.D. degrees (1990) from Rutgers University, New Jersey (USA), all in electrical engineering.He is a University Professor and the Associate Chair for Graduate Studies, Department of Electrical and Computer Engineering, University of Waterloo, Canada. Dr. Shen’s research focuses on resource management, wireless network security, social networks, smart grid, and vehicular ad hoc and sensor networks. Dr. Shen served as the Technical Program Committee Chair/CoChair for IEEE Globecom’16, Infocom’14, IEEE VTC’10 Fall, and Globecom’07, the Symposia Chair for IEEE ICC’10, the Tutorial Chair for IEEE VTC’11 Spring and IEEE ICC’08, the General Co-Chair for ACM Mobihoc’15, Chinacom’07 and the Chair for IEEE Communications Society Technical Committee on Wireless Communications. He also serves/served as the Editor-in-Chief for IEEE Internet of Things Journal, IEEE Network, Peerto-Peer Networking and Application, and IET Communications; a Founding Area Editor for IEEE Transactions on Wireless Communications; an Associate Editor for IEEE Transactions on Vehicular Technology, Computer Networks, and ACM/Wireless Networks, etc.; and the Guest Editor for IEEE JSAC, IEEE Wireless Communications, and IEEE Communications Magazine, etc. Dr. Shen received the Excellent Graduate Supervision Award in 2006, and the Premiers Research Excellence Award (PREA) in 2003 from the Province of Ontario, Canada. He is a registered Professional Engineer of Ontario, Canada, an Engineering Institute of Canada Fellow, a Canadian Academy of Engineering Fellow, a Royal Society of Canada Fellow, and a Distinguished Lecturer of IEEE Vehicular Technology Society and Communications Society.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./Fig/Photo_JieGao.jpg}}]{Jie Gao} (Senior Member, IEEE) received the B.Eng. degree in Electronics and Information Engineering from Huazhong University of Science and Technology, Wuhan, China, in 2007, and the M.Sc. and Ph.D. degrees in Electrical Engineering from the University of Alberta, Edmonton, Alberta, Canada, in 2009 and 2014, respectively. He was a Postdoctoral Fellow with Ryerson University, Toronto, ON, Canada, from 2017 to 2019 and a Research Associate with the University of Waterloo, Waterloo, ON, Canada, from 2019 to 2020. He joined the Department of Electrical and Computer Engineering, Marquette University, Milwaukee, WI, USA, as an Assistant Professor in August 2020. His research interests include machine learning for communications and networking, holistic network virtualization, Internet of Things (IoT) and industrial IoT solutions, and next-generation wireless networks in general. Dr. Gao is an Editor for IEEE Access and Springer Peer-to-Peer Networking and Applications.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./Fig/Photo_WenWu.jpg}}]{Wen Wu}(Member, IEEE) earned the Ph.D. degree in Electrical and Computer Engineering from University of Waterloo, Waterloo, ON, Canada, in 2019. He received the B.E. degree in Information Engineering from South China University of Technology, Guangzhou, China, and the M.E. degree in Electrical Engineering from University of Science and Technology of China, Hefei, China, in 2012 and 2015, respectively. He worked as a Post-doctoral Fellow with the Department of Electrical and Computer Engineering, University of Waterloo. He is currently an Associate Researcher at the Frontier Research Center, Peng Cheng Laboratory, Shenzhen, China. His research interests include 6G networks, pervasive network intelligence, digital twin, and network virtualization. 
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./Fig/Photo_MushuLi.eps}}]{Mushu Li}(Member, IEEE) received the Ph.D. degree in Electrical and Computer Engineering from the University of Waterloo, Canada, in 2021. She received the B.Eng. degree from the University of Ontario Institute of Technology (UOIT), Canada, in 2015, the M.A.Sc. degree from Ryerson University, Canada, in 2017. She is currently a research associate at the Department of Electrical and Computer Engineering at the University of Waterloo. Her research interests include mobile edge computing, system optimization in wireless networks, and machine learning-assisted network management. She was the recipient of NSERC Canada Graduate Scholarships (CGS) in 2018, and Ontario Graduate Scholarship (OGS) in 2015 and 2016, respectively.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./Fig/Photo_ConghaoZhou.jpg}}]{Conghao Zhou}(Student Member, IEEE) received the B.Eng. from Northeastern University, Shenyang, China, in 2017 and the M.Sc. degree from University of Illinois at Chicago, Chicago, IL, USA, in 2018. He is currently working toward the Ph.D. degree at the Department of Electrical and Computer Engineering, University of Waterloo, Waterloo, ON, Canada. His research interests include space-air-ground integrated networks and machine learning in wireless networks.
\end{IEEEbiography}

\vspace*{-1.5\baselineskip}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./Fig/Weihua_Zhuang.jpg}}]{Weihua Zhuang}(Fellow, IEEE) received the PhD degree in electrical engineering from the University of New Brunswick, Canada. She has been with the Department of Electrical and Computer Engineering, University of Waterloo, Canada, since 1993, where she is a University Professor and a Tier I Canada Research Chair in Wireless Communication Networks. Dr. Zhuang is the recipient of 2021 Women's Distinguished Career Award from IEEE Vehicular Technology Society, 2021 Technical Contribution Award in Cognitive Networks from IEEE Communications Society, and 2021 R.A. Fessenden Award from IEEE Canada. She was the Editor-in-Chief of the IEEE Transactions on Vehicular Technology from 2007 to 2013, Technical Program Chair/Co-Chair of IEEE VTC 2017/2016 Fall, Technical Program Symposia Chair of IEEE Globecom 2011, and an IEEE Communications Society Distinguished Lecturer from 2008 to 2011. She is an elected member of the Board of Governors and Vice President for Publications of the IEEE Vehicular Technology Society. Dr. Zhuang is a Fellow of the Royal Society of Canada, Canadian Academy of Engineering, and Engineering Institute of Canada.
\end{IEEEbiography}




==> Final version/Bios.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.3in,clip,keepaspectratio]{./Fig/Xuemin Shen}}]{Xuemin (Sherman) Shen} (Fellow, IEEE)  received the Ph.D. degree in electrical engineering from Rutgers University, New Brunswick, NJ, USA, in 1990. He is a University Professor with the Department of Electrical and Computer Engineering, University of Waterloo, Canada. His research focuses on network resource management, wireless network security, Internet of Things, 5G and beyond, and vehicular networks. Dr. Shen is a registered Professional Engineer of Ontario, Canada, an Engineering Institute of Canada Fellow, a Canadian Academy of Engineering Fellow, a Royal Society of Canada Fellow, a Chinese Academy of Engineering Foreign Member, and a Distinguished Lecturer of the IEEE Vehicular Technology Society and Communications Society. 

Dr. Shen received the Canadian Award for Telecommunications Research from the Canadian Society of Information Theory (CSIT) in 2021, the R.A. Fessenden Award in 2019 from IEEE, Canada, Award of Merit from the Federation of Chinese Canadian Professionals (Ontario) in 2019, James Evans Avant Garde Award in 2018 from the IEEE Vehicular Technology Society, Joseph LoCicero Award in 2015 and Education Award in 2017 from the IEEE Communications Society (ComSoc), and Technical Recognition Award from Wireless Communications Technical Committee (2019) and AHSN Technical Committee (2013). He has also received the Excellent Graduate Supervision Award in 2006 from the University of Waterloo and the Premiers Research Excellence Award (PREA) in 2003 from the Province of Ontario, Canada. He served as the Technical Program Committee Chair/Co-Chair for IEEE GLOBECOM’16, IEEE INFOCOM’14, IEEE VTC’10 Fall, IEEE GLOBECOM’07, and the Chair for the IEEE ComSoc Technical Committee on Wireless Communications. Dr. Shen is the President Elect of the IEEE ComSoc. He was the Vice President for Technical\&Educational Activities, Vice President for Publications, Member-at-Large on the Board of Governors, Chair of the Distinguished Lecturer Selection Committee, and Member of IEEE Fellow Selection Committee of the ComSoc. Dr. Shen served as the Editor-in-Chief of the IEEE IoT JOURNAL, IEEE Network, and IET Communications. 

% received the B.Sc. degree in electrical engineering from Dalian Maritime University, Dalian, China, in 1982, and the M.Sc. and Ph.D. degrees in electrical engineering from Rutgers University, Camden, NJ,
% USA, in 1987 and 1990, respectively.

% He is currently a University Professor from the Department of Electrical and Computer Engineering, University of Waterloo, Waterloo, ON, Canada. His research interests include resource management in interconnected wireless/wired networks, wireless network security, social networks, smart grid, and vehicular ad hoc and sensor networks. 

% Dr. Shen was a recipient of the Excellent Graduate Supervision Award in 2006, the Outstanding Performance Award from the University of Waterloo, in 2004, 2007, 2010, and 2014, the Premier’s Research Excellence Award (PREA) from the Province of Ontario, Canada, in 2003, the Distinguished Performance Award from the Faculty of Engineering, University of Waterloo, in 2002 and 2007, and the Joseph LoCicero Award from the IEEE Communications Society. He served as the Technical Program Committee Chair/Co-Chair for the IEEE Global Communications Conference (GLOBECOM) 2016 and IEEE International Conference on Computer Communications, 2014, the IEEE Vehicular Technology Conference (VTC), 2010, and GLOBECOM’07, the Symposia Chair for the IEEE International Conference on Communications (ICC), 2010, the Tutorial Chair for the IEEE VTC’11 Spring and the IEEE ICC’08, the General Co-Chair for International Symposium on Mobile Ad-Hoc Networking and Computing, 2015, International Conference on Communications and Networking in China, 2007, and International ICST Conference on Quality of Service in Heterogeneous Wired/Wireless Networks, 2006, and the Chair for
% the IEEE Communications Society Technical Committee on Wireless Communications, and P2P Communications and Networking. He also serves/served as the Editor-in-Chief for the IEEE INTERNET OF THINGS JOURNAL, the IEEE NETWORK, Peer-to-Peer Networking and Application, and IET Communications, a Founding Area Editor for the IEEE TRANSACTIONS ON WIRELESS COMMUNICATIONS, and an Associate Editor for the IEEE TRANSACTIONS ON VEHICULAR TECHNOLOGY, Computer Networks, and ACM/Wireless Networks. He is a Registered Professional Engineer of ON, Canada, an Engineering Institute of Canada Fellow, a Canadian Academy of Engineering Fellow, a Royal Society of Canada Fellow, and a Distinguished Lecturer of the IEEE Vehicular Technology Society and Communications Society.
%received the  B.Sc.(1982) degree from Dalian Maritime University (China) and the M.Sc. (1987) and Ph.D. degrees (1990) from Rutgers University, New Jersey (USA), all in electrical engineering.He is a University Professor and the Associate Chair for Graduate Studies, Department of Electrical and Computer Engineering, University of Waterloo, Canada. Dr. Shen’s research focuses on resource management, wireless network security, social networks, smart grid, and vehicular ad hoc and sensor networks. Dr. Shen served as the Technical Program Committee Chair/CoChair for IEEE Globecom’16, Infocom’14, IEEE VTC’10 Fall, and Globecom’07, the Symposia Chair for IEEE ICC’10, the Tutorial Chair for IEEE VTC’11 Spring and IEEE ICC’08, the General Co-Chair for ACM Mobihoc’15, Chinacom’07 and the Chair for IEEE Communications Society Technical Committee on Wireless Communications. He also serves/served as the Editor-in-Chief for IEEE Internet of Things Journal, IEEE Network, Peerto-Peer Networking and Application, and IET Communications; a Founding Area Editor for IEEE Transactions on Wireless Communications; an Associate Editor for IEEE Transactions on Vehicular Technology, Computer Networks, and ACM/Wireless Networks, etc.; and the Guest Editor for IEEE JSAC, IEEE Wireless Communications, and IEEE Communications Magazine, etc. Dr. Shen received the Excellent Graduate Supervision Award in 2006, and the Premiers Research Excellence Award (PREA) in 2003 from the Province of Ontario, Canada. He is a registered Professional Engineer of Ontario, Canada, an Engineering Institute of Canada Fellow, a Canadian Academy of Engineering Fellow, a Royal Society of Canada Fellow, and a Distinguished Lecturer of IEEE Vehicular Technology Society and Communications Society.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./Fig/Photo_JieGao.jpg}}]{Jie Gao} (Senior Member, IEEE) received the B.Eng. degree in Electronics and Information Engineering from Huazhong University of Science and Technology, Wuhan, China, in 2007, and the M.Sc. and Ph.D. degrees in Electrical Engineering from the University of Alberta, Edmonton, Alberta, Canada, in 2009 and 2014, respectively. He was a Postdoctoral Fellow with Ryerson University, Toronto, ON, Canada, from 2017 to 2019 and a Research Associate with the University of Waterloo, Waterloo, ON, Canada, from 2019 to 2020. He joined the Department of Electrical and Computer Engineering, Marquette University, Milwaukee, WI, USA, as an Assistant Professor in August 2020. His research interests include machine learning for communications and networking, holistic network virtualization, Internet of Things (IoT) and industrial IoT solutions, and next-generation wireless networks in general. Dr. Gao is an Editor for IEEE Access and Springer Peer-to-Peer Networking and Applications.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./Fig/Photo_WenWu.jpg}}]{Wen Wu}(Member, IEEE) earned the Ph.D. degree in Electrical and Computer Engineering from University of Waterloo, Waterloo, ON, Canada, in 2019. He received the B.E. degree in Information Engineering from South China University of Technology, Guangzhou, China, and the M.E. degree in Electrical Engineering from University of Science and Technology of China, Hefei, China, in 2012 and 2015, respectively. He worked as a Post-doctoral Fellow with the Department of Electrical and Computer Engineering, University of Waterloo. He is currently an Associate Researcher at the Frontier Research Center, Peng Cheng Laboratory, Shenzhen, China. His research interests include 6G networks, pervasive network intelligence, digital twin, and network virtualization. 
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./Fig/Photo_MushuLi.eps}}]{Mushu Li}(Member, IEEE) received the Ph.D. degree in Electrical and Computer Engineering from the University of Waterloo, Canada, in 2021. She received the B.Eng. degree from the University of Ontario Institute of Technology (UOIT), Canada, in 2015, the M.A.Sc. degree from Ryerson University, Canada, in 2017. She is currently a research associate at the Department of Electrical and Computer Engineering at the University of Waterloo. Her research interests include mobile edge computing, system optimization in wireless networks, and machine learning-assisted network management. She was the recipient of NSERC Canada Graduate Scholarships (CGS) in 2018, and Ontario Graduate Scholarship (OGS) in 2015 and 2016, respectively.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./Fig/Photo_ConghaoZhou.jpg}}]{Conghao Zhou}(Student Member, IEEE) received the B.Eng. from Northeastern University, Shenyang, China, in 2017 and the M.Sc. degree from University of Illinois at Chicago, Chicago, IL, USA, in 2018. He is currently working toward the Ph.D. degree at the Department of Electrical and Computer Engineering, University of Waterloo, Waterloo, ON, Canada. His research interests include space-air-ground integrated networks and machine learning in wireless networks.
\end{IEEEbiography}

\vspace*{-1.5\baselineskip}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./Fig/Weihua_Zhuang.jpg}}]{Weihua Zhuang}(Fellow, IEEE) received the PhD degree in electrical engineering from the University of New Brunswick, Canada. She has been with the Department of Electrical and Computer Engineering, University of Waterloo, Canada, since 1993, where she is a University Professor and a Tier I Canada Research Chair in Wireless Communication Networks. Dr. Zhuang is the recipient of 2021 Women's Distinguished Career Award from IEEE Vehicular Technology Society, 2021 Technical Contribution Award in Cognitive Networks from IEEE Communications Society, and 2021 R.A. Fessenden Award from IEEE Canada. She was the Editor-in-Chief of the IEEE Transactions on Vehicular Technology from 2007 to 2013, Technical Program Chair/Co-Chair of IEEE VTC 2017/2016 Fall, Technical Program Symposia Chair of IEEE Globecom 2011, and an IEEE Communications Society Distinguished Lecturer from 2008 to 2011. She is an elected member of the Board of Governors and Vice President for Publications of the IEEE Vehicular Technology Society. Dr. Zhuang is a Fellow of the Royal Society of Canada, Canadian Academy of Engineering, and Engineering Institute of Canada.
\end{IEEEbiography}




==> Final version/sec_Challenges_and_Open_Issues.tex <==
%\subsection{Open Issues}
%1. modeling-Relationship between required resource and achieved performance for AI services is unclear; 2. configuration- scheduling decision for inference slice; 3. joint resource allocation for trianing slice and infernece slice; 4. GPU-CPU heterogeneous architecture； 4. New AI technologies for resource limited wireless networks, such as DNN model compression (computing), data compression(communication), model partition (computing), co-inference (computing), data-importance transmission, transfer learning, 

Many challenges and open issues are yet to be addressed for holistic network virtualization and pervasive network intelligence in 6G. In the following, we present some key challenges and open issues.

%The research in these two fields is still in its infancy stage, and a great deal of open issues need to be carefully solved before practical implement. In the following, we summarize some of the challenging research issues.  

\subsection{Digital Twin}

The six-layer architecture in Subsection~\ref{ss:HNV} provides a high-level design for integrating the digital twin paradigm into network virtualization. Open issues to be investigated for practical implementation of this architecture include quantitative performance characterization of digital twins, the optimal digital twin model, digital twin migration, and data security. 

First, it is necessary to quantitatively characterize the network performance improvement from introducing digital twins, either from the perspective of QoS/QoE satisfaction or from the perspective of resource utilization. %With such quantitative performance characterization, the network would be able to search for the optimal digital twin model. 
Second, level-one digital twin models configured by the centralized controller may be different for different edge networks to account for network heterogeneity, and how to determine effective digital twin models is a challenge. Third, the mobility of end users such as vehicles creates a need for updating and migrating digital twins across different edge networks, which requires further study. 
%The aforementioned difference in digital twin data models at different edge networks may further complicate the migration. 
Last, ensuring the security of user data in the digital twin paradigm is yet another challenge. As the local and centralized network controllers have access to a vast amount of user data, developing proper security mechanisms for data collection, aggregation, and migration becomes essential. Readers are referred to \cite{J_RMinerva_ProcIEEE_2020,J_YLu_IoT_2021,J_WJiang_OJCS_2021,J_PBellavista_TII_2021} for discussions on some of the aforementioned challenges, such as the heterogeneity and migration of digital twins, and more open issues related to digital twins in 6G.
       
\subsection{Network Management Oriented Data Abstraction and Processing}

While digital twins provide data to enable AI for networking, including automated network slicing and AI-empowered network control, efficient data management can be challenging. First, it is necessary to develop data abstraction methods to aggregate the data with different levels of granularity for making different network management decisions. For instance, in network slicing, high-granularity data are required for determining the optimal network operation strategies and low-granularity data are sufficient for determining the optimal network planning strategies~\cite{J_XShen_2020,Mei}. How to determine the appropriate data granularity for different network management decisions is an open issue. 
A potential solution is to empirically adjust data granularity and the time scale for decision-making \cite{Marquez}. Meanwhile, as the number of variables and data types in network management can be huge, more scalable and efficient solutions are required. 
Second, while applying the connected AI solution for network management, the settings of intelligent modules, such as the selection of  algorithms, the input and output attributes, and the connections among intelligent modules, should be configured to maximize the utilization of data with low communication and processing overhead, yet finding the optimal settings is challenging. The cooperation between model-driven and data-driven methods in intelligent modules can be a potential approach to address the challenge, yet how to support such cooperation among different types of intelligent modules requires further investigation. Third, as data can be generated, transmitted, and processed at different network stakeholders, configurable and regulation-compliant data management is also a challenge. The integration of the blockchain and privacy-enhancing technologies can be a potential solution, while the trade-offs between privacy preservation and processing efficiency need in-depth investigation. Readers are referred to \cite{MNet_XShen_2020, zhou2019edge, wu2021ai, S_DC.Nguyen_ST_2021} for discussions on the aforementioned challenges, such as privacy preservation, AI model selection, intelligent modules, and more open issues about data abstraction and processing.


\subsection{Model and Resource Orchestration}
% \textcolor{blue}{This subsection title is too big}
Networking for AI in Subsection~\ref{ss:NetforAI} can facilitate AI services in a network. One key issue is to optimize AI service performance, which requires judicious configuration of the network, including AI algorithm selection, data collection, and network resource allocation. The main challenge lies in modeling the relationship between AI performance and these network configurations. Establishing an accurate mathematical or empirical model requires extensive measurements in real-world networks. Even if establishing a model is viable, the  model may be suitable only for a chosen AI algorithm. In addition, to adapt to network dynamics (e.g., rapidly fluctuating service demands), an online network configuration scheme is desirable. Since reinforcement learning algorithms are able to make online decisions in a dynamic environment, developing cost-effective reinforcement learning algorithms for high-dimensional network configuration problems can be a promising approach. For example, a reinforcement learning algorithm is developed for joint AI model selection and resource allocation in industrial IoT~\cite{wu2020accuracy}. For more discussions on the above challenges, interested readers are referred to~\cite{partition1, partition2, he2020optimizing}. 

% Reinforcement learning (RL) based algorithms hold the potential to deal with the online decision making problem. However, purely relying on a vanilla RL algorithm is challenging in practical systems. The reason is two-fold. Firstly, obtaining the optimal multi-dimensional configuration requires voluminous training data and prohibitively long training time, which challenges applicability in fast-changing networks with limited training data. Secondly, the amount of consumed network resources of executing some configurations can be orders of magnitude higher than the most efficient one. Hence, cost-efficient and fast RL algorithms are imperative. This can be approached via hybrid data\&model driven methods, as mentioned in Section~\ref{subsec:Model-data Co-driven}, which leverages the domain knowledge provided by constructed coarse models to speed up training process while requiring a small amount of training data.


%
\subsection{Training and Inference Coordination} 
The concept of AI slice is proposed to meet specific QoS requirements of AI services in Subsection~\ref{ss:NetforAI}. The training and inference stages for an AI service consume multi-dimensional network resources~\cite{lin2019artificial, zhou2019edge}. In an AI slice, two subslices share the virtualized network resource pool, and hence resource reservation decisions for the two subslices are closely correlated. On the one hand, reserving abundant resources for the training subslice may help achieve a high training accuracy but potentially render resource insufficiency in the inference subslice, which can result in a long service latency. On the other hand, insufficient resource provisioning for the training subslice may yield a model with low accuracy and consequently create a bottleneck for inference accuracy. To optimize the performance of the AI service, resource reservation for training and inference subslices should be coordinated. Developing an accurate mathematical model to characterize the interplay between training and inference stages is difficult, since a large number of system factors should be taken into account. Hence, it is necessary to study efficient model-free approaches to characterize the interplay. 
% In addition, abstracting and characterizing the impact of data-related factors in wireless networks, such as data availability, data importance, and data distribution, remain an unexplored research area.

%for the optimal resource orchestration, by taking many factors into account. 


\subsection{Energy Efficiency of AI}
% AI services are computation-intensive in both the training and the inference stages, which could incur prohibitive energy consumption at energy-constrained end users and network edge.
With hundreds of neural network layers, thousands of neurons, and millions of parameters, state-of-the-art AI models usually consume extensive energy and incur substantial environmental costs.\footnote{The estimated carbon footprint of training a state-of-the-art natural language processing model is about five times the life emissions of an average car~\cite{strubell2019energy}.} Improving energy efficiency has become a major issue for  wide deployment of AI services.  In addition, recent research shows that improving the accuracy of an AI model may come at an exponential increase in the computation, environmental and economic costs~\cite{thompson2020computational}.\footnote{It is estimated that reducing the classification error probability from 11.5\% to 5\% over the ImageNet dataset needs to increase computation from 10$^{14}$ to 10$^{19}$\;Gflops, carbon emissions from 10$^6$ to 10$^{10}$\;lbs, and economic costs from 10$^6$ to 10$^{11}$\;USD~\cite{thompson2020computational}, respectively.} Hence, deploying energy-efficient AI services in a network is necessary for reducing costs for the network operator and meeting environmental standards. Several model compression techniques, such as weight pruning~\cite{han2015deep}, parameter quantization~\cite{zhu2016trained}, and model compression\cite{hinton2015distilling}, can be applied to alleviate the problem. %Since model performance is sacrificed in these schemes, the main challenge lies in balancing the model performance and energy consumption.  
In addition, hybrid data-model driven methods can train AI models with a reduced amount of data, which can also decrease energy consumption.


\subsection{Hybrid Data-Model Driven Methods}

The four options listed in Subsection~\ref{ss:codriven} provide our initial ideas for hybrid data-model driven methods. Related open issues to be investigated include the following. First, it is necessary to study how to determine which option to use and how to switch among options. Designing mechanisms for choosing and switching among options will allow networks to flexibly and adaptively integrate data-driven and model-driven methods. Second, for a chosen option, it is important to understand how much the data-driven and model-driven components affect the overall performance and how much impact they have on each other. For instance, in the mixing option, the AI service performance may depend on the combined choices of data-driven and model-driven methods, and finding a proper combination can be a challenge. Third, in addition to the four options as introduced, there should be other potential options for hybrid data-model driven methods, and identifying other promising options is an open issue of great importance. Last, due to the lack of explainability in existing data-driven methods, careful investigations and analysis should be directed to the management of critical network operations. The role of hybrid data-model driven methods in enhancing system robustness is an open issue that deserves further investigation. For more discussions on challenges in hybrid data-model driven methods for networks, interested readers are referred to \cite{zappone2019wireless, M_CWang_WCom_2020, M_TWang_ChinaCom_2019}.\footnote{ An application of a hybrid approach in vehicular network simulation can be found in \cite{C_BSliwa_GC_2020}.  }




%By analysing 1,058 research papers on deep learning, a very recent work shows 


%\subsection{Others}
%There are some other open issues should also be investigated in the future, which are listed as follows. DL specific computation facilities, such as graphics processing unit (GPU) and tensor processing unit (TPU), have been widely applied in cloud-based AI systems, which will be extended and integrated with existing central processing unit (CPU) computation facilities in wireless networks. To further unleash learning power, how to coordinated heterogeneous computing facilities for different types of ML tasks is a novel and important problem. In addition, it is not bold to think that most existing model-based control modules in 6G networks are replaced by AI-based ones.  Large-scale network operation  requires joint decision making via multiple AI-based control modules,  which may cause non-stationary issue. The possibility of potential divergence issues occur requires further investigation and backup design.

==> Final version/sec_Holistic_Network_Virtualization.tex <==
%Virtualization has become an important trend in modern wireless networks. 
In this section, we first review virtualization techniques in existing networks and their benefits. Then, we introduce the idea of holistic network virtualization.  

\subsection{Network Virtualization}\label{ss:NetVirtual}

The concept and techniques of network virtualization have been evolving over more than three decades~\cite{M_Mosharaf_COMM_2009}. Early research on network virtualization includes virtual local area networks motivated by facilitating different types of operations (services) in distributed systems~\cite{rossi1986proposal}, as well as providing flexible network control and improving link utilization~\cite{J_KSato_TCOM_1990}.  Another example of network virtualization is virtual private networks, which establish efficient and secure communication links to connect geographically dispersed end users. Over time, the desire for programmable network management extends to the objective of enhancing network architecture.    

The advancement in cloud computing has propelled recent development in network virtualization, including network function virtualization (NFV) and network slicing. With NFV, software instances running on virtual machines at general computing servers replace customized and proprietary hardware for various network functions~\cite{J_KQu_TCom_2020}. At the network core, NFV applies to functions such as switching, firewall, deep packet inspection, and session border controller~\cite{C_chioC_2012}. At radio access networks, NFV applies to frame generation, modulation, carrier allocation, etc.~\cite{J_AGDalla-Costa_JSAC_2020}. The realization of NFV becomes an enabler for network slicing, which is a key network architecture innovation in 5G. Network slicing emphasizes a service-oriented perspective in network management by creating multiple end-to-end virtual networks, i.e.,  slices, for different services on top of shared physical network infrastructure. With network slicing, network resources are first reserved for respective services in network planning stages and later allocated to individual users in network operation stages~\cite{J_XShen_2020}. The creation, adjustment, and termination of slices are based on the varying spatiotemporal distribution of service demands to provide a high level of flexibility and adaptivity in network management~\cite{J_HZhang2016}.\footnote{SDN and C-RAN are also closely related to network virtualization since virtualization significantly simplifies and expedites their realization in modern wireless networks.} 


Virtualization can be applied on different levels and scales in a network. Existing techniques include virtualization at \emph{node, link, resource}, and \emph{network} levels. Virtual nodes are abstractions of substrate nodes in a network such as servers, routers, and switches, and typical examples of node virtualization are storage and computing server virtualization \cite{J_GZhang2007}, \cite{J_FXu_2014}. Virtual links are the logical channels that interconnect virtual nodes. Virtual resources are abstractions of computing, memory, storage, and communication resources in a network~\cite{J_PBellavista_2019}, while physical resources at different locations can form virtual resource pools~\cite{J_KQu_TCom_2020}. For instance, the virtualization of a network function is the execution of a network control or service function by running software, supported with necessary resources. A virtual network is the combination of virtual nodes and links with proper virtual resource allocation for a service request to meet its QoS requirements, supported by necessary networking protocols. Besides the aforementioned works, more representative research works on node, link, resource, and network virtualization are summarized in Table~\ref{Table:NetVirtual}.



\begin{table*}[hbt!]
	\centering
\scriptsize{
	\caption{Some Representative Works on Node, Link, Resource, and Network Virtualization}\label{Table:NetVirtual}
\begin{tabularx}{0.92\textwidth}{|p{1.5cm}|l|p{2.5cm}|p{3cm}|X|}
\hline
\textbf{Type}    &  \textbf{Work}  & \textbf{Scenario} &  \textbf{Research Focus} & \textbf{Objective} \\ \hline
\multirow{10}{*}{\parbox{2cm}{Node \\Virtualization}} & \cite{J_XYuan2021} & Edge computing & Virtual edge node placement & Low-cost placement and fast response to user requests \\ \cline{2-5}
 & \cite{J_SYang2017} & Cloud computing & Virtual machine (VM) placement  & Reliable VM placement and routing \\ \cline{2-5}
 & \cite{J_MNagy_2018} & IP network & Virtual node/router as IP overlay & Practical IP-level resilience to link failures \\\cline{2-5}
 & \cite{M_Khan2015} & Wireless sensor network (WSN) & Architecture for sensor virtualization in WSN & Multiple applications share the same WSN  \\\cline{2-5}
 & \cite{J_SZaidi_2019} & C-RAN & Clustering of access points & Forming user-specific virtual base stations given QoS requirements \\
 \hline
\multirow{6.5}{*}{\parbox{2cm}{Link \\Virtualization}} & \cite{J_HDu2013} & WSN & Virtual backbone construction  & Enabling low-complexity backbone construction with performance guarantee  \\ \cline{2-5}
& \cite{J_FHosseini_2019} & Generic & Virtual link embedding & Reducing congestion probability given bandwidth demands \\ \cline{2-5}
&\cite{J_STomovic2019} & Internet service provider (ISP) network with SDN & Virtual link provision &  Maximizing network throughput subject to QoS and robustness constraints \\\cline{2-5}
\hline
\multirow{13}{*}{\parbox{2cm}{Resource \\Virtualization}} & \cite{J_CPapagianni_2013} & \multirow{2}*{Cloud computing}  & Composite virtual resource mapping  & Efficient mapping of computing and networking resources to substrate resources within
networked clouds  \\ \cline{2-5}
& \cite{J_TWood2015} & Cloud computing & VM migration & Low-cost transferring of VM storage and 
memory during VM migration over wide area networks \\ \cline{2-5}
&\cite{L_MKali_2016} & Radio access network (RAN) & Radio resource virtualization &  Maximizing throughput with fairness among multiple mobile network operators \\\cline{2-5}
&\cite{J_XLu_2019} & RAN & Radio resource virtualization &  Delay-bounded QoS provisioning through radio resource virtualization \\\cline{2-5}
& \cite{J_SZhang2020} & Vehicular network & Resource sharing among slices  & Reusing communication and caching resources to support applications with different QoS requirements \\ \cline{2-5}
\hline
\multirow{13}{*}{\parbox{2cm}{Network \\Virtualization}}  & \cite{J_OAlhussein_2020} & 5G core network with SDN & Network function chain embedding & Minimizing embedding cost subject to network resource constraints \\ \cline{2-5}
& \cite{J_NZhang_2017} & Core network with SDN & Network function chain embedding &  Minimizing total flow in the network subject to network resource constraints \\ \cline{2-5}
& \cite{J_JTang2019}  & C-RAN & Slice request admission &  Maximizing the revenue of the C-RAN operator subject to network resource constraints \\ \cline{2-5}
& \cite{J_QYe2018}  &  Heterogeneous wireless network &  Dynamic radio resource slicing &  Maximizing network utility through optimal bandwidth slicing and user association \\ \cline{2-5}
& \cite{J_TGuo2019}  & 5G RAN &  Radio resource allocation in RAN slicing &  Satisfying QoS requirements by proper resource mapping and scheduling \\ \cline{2-5}  
& \cite{J_JNi2018} & IoT & Service-oriented authentication & Privacy-preserving slice selection and secure access of service data \\
\hline
\end{tabularx}
}
\end{table*}

Regardless of its level and scale, virtualization in the context of networking typically demonstrates the following characteristics:
\begin{itemize}
	\item Abstraction - Abstraction provides a high-level overview of a network while hiding details of the underlying physical network entities (nodes, links, or networks) or resources~\cite{J_MKessler_2008}. This simplifies network management and facilitates flexible service provision; 
	\item Co-existence - Multiple virtual entities corresponding to a shared physical entity co-exist, or multiple virtual resource pools co-exist on the same physical resource pool~\cite{M_Mosharaf_COMM_2009}. This enables service-oriented virtual networks and improves network resource utilization efficiency;
	\item Isolation - Coexisting virtual entities corresponding to the same physical entity should function independently~\cite{S_JVBelt_2017}. This is necessary for guaranteeing service reliability, security, scalability, and QoS satisfaction.     
\end{itemize}    

Both academia and industry have spent a significant amount of efforts on network virtualization. For virtualizing core networks, some works leverage SDN techniques to separate the control and data planes through different protocols or application programming interface (API), e.g., OpenFlow~\cite{mckeown2008openflow}. Furthermore, network virtualization has been extended to radio access networks (RANs), and several frameworks for RAN virtualization are proposed. A SoftRAN framework enables both centralized and distributed RAN control based on the time sensitiveness of control decisions~\cite{gudipati2013softran}. Another framework, FlexRAN, offers a hierarchical architecture for real-time RAN control and incorporates a flexible  API to separate control and data planes in RANs~\cite{foukas2016flexran}. Initiated by industry, such as AT$\&$T and China Mobile, Open-RAN (O-RAN) is proposed as an open-source and open-interface platform to support RAN virtualization~\cite{ORAN}, which can incorporate AI and provide APIs for data-driven networking~\cite{breen2021powder,johnson2021open,foukas2021concordia}.

The adoption of virtualization techniques renders modern networks programmable, flexible, and scalable, which significantly increases cost effectiveness in network deployment and operation. Due to these benefits, it is foreseeable that advanced virtualization techniques will be essential to 6G. Meanwhile, the existing scope of network virtualization is limited in the sense that virtualization techniques mostly focus on network infrastructure and resources, yet less attention is given to end users. In 6G, end user virtualization will become necessary for two reasons. First, with increasingly diverse end user devices, resource-demanding services, and heterogeneous and dynamic networks, providing QoE guarantee for end users will become more challenging in the era of 6G. Accurate characterization and abstraction of end users, which necessitate end user virtualization, can be a precondition to QoE satisfaction. Second, as AI will be a highlight of 6G, extensive user data are required to fuel AI services and AI-based network management. Given such need for data, end user virtualization can be a competitive approach for collecting, managing, and processing data from end users.   





%Virtualization focuses on different levels, including node, link, resource (NFV), and network. 
%
%Virtualization first gained momentum in computing. 
%
%abstraction -- separation (virtual machine/network from physical infrastructure) 
%
%isolating different virtual machines network, guarantee QoS
%
%sharing -- improve resource utilization through multiplexing among different virtual machines/networks


%fundamental motivation for virtualization: programmable/re-configurable/shareable for increased network hardware/resource utilization and reduced cost.
%
%reduce the cost of network deployment and operations
%
%Cloud-RAN sharing BBU
%
%NFV - Core side, RAN side
%SDN - control logic virtualization
%cloud ran? (RAN side network virtualization)
%Network slicing (RAN and/or Core)

\subsection{End User Virtualization}~\label{ss:EUVirtual}

 Until recently, only a few works study end user virtualization in the context of networking. One early example relevant to end user virtualization is network-hosted avatars, i.e., virtual agents, of end users for applications such as file downloading when the users are offline~\cite{J_AConte_2008}. Another example is virtual objects, proposed as a component in Internet of things (IoT) platforms~\cite{S_MNitti_2016}. The motivation is to handle the heterogeneity of physical objects (end users) via virtualization and to facilitate the provision of services to end users.  

%, e.g., virtual sensors~\cite{C_KAberer_2007}.

% Lately, \emph{digital twin} starts to attract attention in the field of IoT. Originated in the manufacturing industry, the term ``digital twin" is characterized by full digital representation of physical objects or processes and real-time synchronization between the physical objects and their corresponding digital replicas~\cite{W_MGrieves_2014, khan2021digital}.  
As a potential paradigm to enable end user virtualization, digital twin attracts much attention lately. The concept of digital twin was originally conceived by Michael Grieves for product life-cycle management in industry in 2003~\cite{W_MGrieves_2014, khan2021digital}. Later, NASA and U.S. Air Force Vehicles developed a digital twin paradigm for vehicles to forecast their remaining usable life and the mission success probability~\cite{ glaessgen2012digital}. A digital twin is characterized by a full digital representation of a physical object or a process and real-time synchronization between the physical object or process and its corresponding digital replica. Digital twins can contain a large volume of data from physical objects or processes for advanced analytics, and the analytical results can be used to improve the performance of the corresponding physical objects or processes. Exemplary digital twins in general application scenarios, as well as potential requirements for the digital twins to enable big data analytics, are discussed in~\cite{TII_Gao}. Potential implementation of digital twins representing IoT devices in  industrial systems is proposed in~\cite{madni2019leveraging}. Other representative research works on digital twins are summarized in Table~\ref{Table:DigTwin}. 

Most existing research on digital twins in the network field focuses on applications, e.g., distributed clock synchronization~\cite{J_PJia_2020} and computation offloading \cite{J_YDai_2020}. In comparison, the study of digital twins from the perspective of network architecture and network management is limited at the moment.\footnote{Some works focus on distributed networks, e.g., vehicular networks, and adopt digital twins as an approach for network virtualization instead of end user  virtualization~\cite{M_LZhao_2020},\cite{C_JTaylor_2020}.} A digital twin based cloud-centric network architecture is proposed in~\cite{M_Q_Yu_2019}, where digital twins of end users hosted at the network edge play the role of communication assistants or network data loggers. 
% \textcolor{purple}{A configurable digital twin framework is designed for vehicular network management, where digital twins provide extensive vehicle information to facilitate AI-based radio resource allocation~\cite{TVT_Zhou_2021}.} 

%The integration of digital twin into software-defined vehicular network is proposed in \cite{M_LZhao_2020}, highlighting a comparison of different routing schemes in different    the predict and simulation  




\begin{table*}[hbt!]
	\centering
\scriptsize{
	\caption{Some Related Works on Digital Twins}\label{Table:DigTwin}
\begin{tabularx}{1\textwidth}{|l|p{2.3cm}|p{2.3cm}|p{4cm}|X|}
\hline
 \textbf{Work}  & \textbf{Application } & \textbf{Type of Physical Object} & \textbf{Role of Digital Twin} &  \textbf{Target of Using Digital Twin}\\ \hline
 \cite{J_ABarbie_2021} &  Underwater network for ocean observation & Underwater sensors/actuators & Monitoring and testing observation system & Visualizing an ocean observation system and enhancing simulations\\  \hline
 \cite{J_XXu2020} &   Edge computing for internet of vehicles & Vehicles & Collecting and sharing information about vehicles and surroundings & Empowering computing offloading by facilitating data analytics  \\  \hline
 \cite{J_HWang2020} &   5G network slicing & Network slices & Predicting and monitoring slice performance & Assisting autonomous network slicing \\  \hline
 \cite{J_TWang2020} &   Smart factory & Workstations in a conveyor system & Evaluating and validating control strategies
 & Implementing intelligent conveyor systems \\  \hline
\cite{M_OEMarai2020} &   Smart city & Road infrastructure & Monitoring roads and detecting vehicles/persons
 & Supporting smart city applications through gathering and processing data \\  \hline
\cite{J_RMinerval_2021} & IoT  &  Objects with sensing capability & Storing data for detecting events and recognizing behaviors & Facilitating synthetic sensing through situation awareness and explainability \\  \hline
\cite{J_ACastellani2020} &   Industry 4.0 &  Industrial machinery & Generating training dataset and simulations & Achieving accurate anomaly detection with limited labelled data \\  \hline
\cite{J_HElayan2021} &  Smart healthcare &  Patients  & Handling data for analysis and developing AI models & Improving healthcare operations \\  \hline
\cite{J_MSchluse2018} &  Industry 4.0 &  Technical assets (e.g., machine, environment)  & Integrating knowledge from model and data for simulations & Enhancing simulation-based systems engineering \\  \hline
\cite{J_RDong2019} &  Mobile edge computing &   Real-world network environments  & Training learning algorithms and monitoring network environments &  Enabling learning for optimizing user association, resource allocation, and
offloading \\  \hline
\cite{J_CGehrmann2020} &  Industrial 4.0 &  Products, workstations, conveyor belts  &  Data sharing
and control of security-critical processes &  Building a security architecture based on state replication and synchronization \\  \hline
\cite{J_KMAlam2017} &  Cyber-physical systems &   Generic physical devices  &  Monitoring, diagnostics, and prognostics  & Supporting applications such as context aware interaction and driving assistance \\  \hline
\cite{J_LFRivera2021} &  IoT &   Generic physical systems  &  Managing context information and self-adapting & Increasing  autonomy and enhancing cooperation through autonomic digital twins \\  \hline
\cite{zhang2020manufacturing} &  Welding manufacturing &  Human-robot interaction systems  &  Monitoring welding robot and enabling simulations & Visualizing  welder behavior and training welders \\  \hline
\cite{fang2019digital} &   Smart manufacturing &   Job shop scheduling systems  &  Obtaining scheduling data and simulating scheduling strategies & Enabling timely response and reducing scheduling plan deviation \\  \hline
\cite{xu2019digital} &  Smart manufacturing &   Manufacturing systems  &  Predicting and verifying the system performance & Increasing  autonomy and enhancing fault diagnosis \\  \hline
\cite{jain2019digital} &  Smart building &  Photovoltaic energy conversion units  &  Estimating the status of photovoltaic energy conversion unit & Improving the accuracy of fault detection \\  \hline
\cite{IOT_Sun_2021} &  Internet of vehicles &  Vehicles and road side units  &  Monitoring the real-time status of vehicles and road side units & Supporting network resource management  \\  \hline
\cite{TCSS_Zhang_2021} &  Mobile edge caching &   Vehicles  &   Capturing the social characteristics of vehicles & Improving the effectiveness of cache management \\  \hline
\end{tabularx}
}
\end{table*}


Digital twin appears to be an intuitive solution to end user virtualization. Nevertheless, extending the existing network virtualization, represented by network slicing, to end users is not straightforward, given the target of flexible and efficient network management and service provision. For instance, it is trivial to simply use node-level virtualization and to represent end users as virtual data sources or sinks in a virtual network. Moreover, while end users may possess communication and computing resources, resource-level virtualization does not characterize user-specific properties, e.g., location and mobility, or service-specific properties, e.g., data traffic variations, of end users. It is necessary to understand potential \textit{benefits, requirements}, and \textit{implementation} of digital twin based end user virtualization, with a particular focus on the integration of digital twin and existing network virtualization frameworks.  

There are potentially two-fold \textit{benefits} of digital twin based end user virtualization, i.e., extensive end user data and powerful network emulation capability. While the virtualization of network infrastructure and resources characterizes the network status and \textit{service provision} capabilities, digital twins of end users can provide extensive data regarding \textit{service demand} and user QoS/QoE satisfaction. Such data can play a significant role in network management through facilitating well-informed network planning and operation decisions. Moreover, the real-time or near real-time synchronization between end users and their digital twins enables powerful network emulations. For instance, multiple instances of the same virtual network can be created, with real-time end user information, e.g., location and data traffic volume, provided to all instances through synchronized end user digital twins.\footnote{The emulation can apply to a virtual network segment, e.g., the network edge.} Different network planning or operation strategies can be applied and emulated in different instances, while each instance remains synchronized with the real-world network environment through the information provided by the digital twins of end users.    



%parallel and partially synchronized emulations for evaluating network management or service provision strategies. For example, multiple virtual network instances can be created in the cyber space, each for testing a specific strategy, while the real-time location or data traffic volume of users are reflected in all instances. 

%key challenge: embedding - synchronization

To take part in network virtualization, digital twins of end users should satisfy the following \textit{requirements}:
\begin{itemize}
	\item Flexible: The abstraction of end users into digital twins must be sufficiently flexible to represent heterogeneous physical devices (such as smartphones, vehicles, and industrial sensors) and serve various applications (such as virtual reality gaming, autonomous driving, and industrial automation); 
	\item Compatible: The end user virtualization based on digital twins should complement and enhance the state-of-the-art network virtualization, i.e., network slicing. For instance, digital twins of end users should provide data to support various network slices, while each slice may only have access to a subset of data pertinent to that slice;      
	\item Customizable: The attributes of digital twins should be customized and updated based on the corresponding service, network traffic, resource utilization, etc. For instance, the amount and types of data included in a digital twin should be adaptable rather than fixed. In addition, while the focus of digital twins is placed on end users, digital twins should be able to represent other network entities, e.g., unmanned aerial vehicle (UAV) mounted mobile base stations (BSs). 
\end{itemize}
In addition, network resource consumption from creating and maintaining digital twins should be taken into account.

Noting the aforementioned benefits and requirements, we aim to answer the following key questions with respect to the \textit{implementation} of digital twins: 
%Last but not least, the followings are key \textit{implementation} issues regarding digital twin, which must be appropriately addressed:
\begin{itemize}
	\item Location: Where should digital twins be hosted in a network? % Who maintains the digital twins? %not necessarily every node, depending on QoS, privacy settings, representative, location, etc.
	\item Affiliation: Should digital twins exist within or outside  network slices? 
	\item Data: What data attributes pertinent to networking should be included in a digital twin? How much historical data should be included for a specific attribute? Should predicted user information be included?
	\item Synchronization: How to determine the frequencies of updating various data entries of a digital twin by acquiring new data from the physical object?     
	\item Control: Who should determine and update digital twin models and based on what information?
%	\item How to customize
%	\item Recursion across levels
%	\item Access limits
%	\item exits within or outside of slices
\end{itemize}
In the next subsection, we propose a novel conceptual architecture for holistic network virtualization, which integrates digital twins and network slicing, and delve into the above questions.  




%Difference with digital twin in industrial 
%\begin{itemize}
%	\item all physical properties vs. properties pertinent to networking
%	\item one to one \cite{J_MSchluse_2018} vs. one to many
%	\item migration/multihoming
%\end{itemize}

%Usage of digital twin
%\begin{itemize}
%	\item Monitoring and prediction
%	\item Emulations/Tests for comparing strategies numerically
%	\item Decision making (through providing data)
%\end{itemize}


 \begin{figure*}[tt]
	\centering
	\renewcommand{\figurename}{Fig.}
	\includegraphics[width=1\textwidth]{Fig/fig1.pdf}
	%	\vspace{0cm}
	\caption{The conceptual six-layer virtualization architecture for holistic network virtualization.}
	\label{fig:digital_twin}
\end{figure*}

\subsection{Holistic Network Virtualization}\label{ss:HNV}



We propose a novel virtualization architecture, i.e., holistic network virtualization, for integrating digital twins into network virtualization, in order to improve network management and service provision capabilities. The proposed virtualization architecture consists of six layers and is illustrated in Fig.~\ref{fig:digital_twin}, in which virtualization layer (VL)~1 is the bottom layer for data collection and VL~6 is the top layer for digital twin model control. The outline of each layer is given as follows:

%\begin{itemize}
	%\item 
	\textit{VL~1 -- Data Collection}: Data required for the digital twin representation of selected end users are collected from the corresponding physical entities following prescribed data precision, uploading method, collection frequency,~etc. The data are collected via access points, and the data collection is controlled by local controllers deployed at network edge; 
	%\item 
	
	\textit{VL 2 -- Level-One Abstraction}: Based on the current \textit{digital twin model} from the digital twin model control layer (i.e., VL 6), which determines the content and format of data included in every digital twin, digital twins are formed and updated using data collected by VL~1. The abstraction may include the aggregation of data from different sources, the update of historical data, and the creation of digital twins for new or additional end users. The digital twins created in this layer are \textit{level-one digital twins}, representing individual end users, and hosted at servers connected to local controllers;
	
	%\item 
	\textit{VL 3 -- Local Processing and Control}: The data from level-one digital twins are processed at network edge for predicting behaviors of individual users, such as user data traffic and mobility patterns, and making user-level service decisions, such as computing offloading, content delivery, and link-layer protocol adaption. Local processing may also include emulations of an edge network or a part of it based on level-one digital twins. Local control may include further data aggregation from level-one digital twins for VL~4, the migration of digital twins based on user mobility, and the selection of end users for digital twin representation. Similar to the case of VL~2, the local processing and control occur at servers affiliated with local controllers; 
	
	%\item 
	\textit{VL 4 -- Level-Two Abstraction}: The aggregated data from VL~3 is sorted into service-specific data for respective network slices in VL~4. Additional data that describe slice configuration, slice resource utilization, slice service level agreement satisfaction, etc., are generated for each slice. Then, the aforementioned data are abstracted to form or update the digital twins of various slices. The digital twins created in this layer are \textit{level-two digital twins}, which are associated with virtual networks (slices). The level-two digital twins are hosted at servers connected to the centralized controller of the network;
	
	%\item 
	\textit{VL 5 -- Slice-Level Processing and Control}: The data from level-two digital twins of network slices are processed for service-specific prediction, e.g., spatiotemporal service demand distribution forecast, or slice-level decision making, e.g., planning and operation decisions. Slice-level processing may include emulations of an end-to-end slice or a part of it based on level-two digital twins. Slice-level control may include slice admission, resource reservation, and slice service coverage control. Similar to the case of VL~4, the service-level processing and control occur at servers affiliated with the centralized controller of the network; 
	
	%\item 
	\textit{VL 6 -- Digital Twin Model Control}: This layer determines and updates the models of level-one and level-two digital twins based on  available network resources for digital twins, the performance of network management and service provision decisions derived based on the current digital twins, and the dynamic spatiotemporal service demands. For instance, VL~6 determines data precision, synchronization frequencies for different data attributes, the amount of historical data contained in the digital twins for each attribute, and the inclusion of predicted user information. In addition, this layer decides the subset of data in level-one digital twins that each slice can access. The digital twin model control also occurs at servers affiliated with the centralized controller of the network;
%\end{itemize} 

The level-one digital twin model configured by VL~6 may include the following data, which shall be collected by the local controllers from end users at VL~1: (1) connectivity and channel information, such as the AP(s) that an end user is connected to and the channel state information for each connection; (2) service information, such as active service types, data traffic volume of each service, and QoS satisfaction of each service; (3) user information, such as user profile, user location and mobility, network resources allocated to the user, and the local computing and caching capabilities of the user; and (4) additional use case-specific information, such as motion sensor readings for augmented reality interactive gaming or operation log for industrial IoT devices. The level-two digital twin model configured by VL~6 may include the following data, which shall be collected or generated by the centralized controller: (1) slice service demand, such as the number of service requests and the spatiotemporal service request distribution; (2) slice resource configuration, such as the reserved communication, computing, and caching resources for the slice; (3) slice performance, such as the slice service level agreement satisfaction, slice resource utilization, and slice energy consumption; (4) slicing strategy, such as the method or algorithm used for network function deployment, resource reservation, and resource scheduling; (5) additional use case-specific information, such as UAV trajectory configuration for UAV-assisted networks. Note that different end user digital twin models are applicable to different types of end users, and each network slice may have a uniquely defined slice digital twin model. For example, the digital twins of vehicles and industrial IoT devices most likely contain different data, and the digital twin models may differ between slices for industrial IoT and those for smart home or between slices of different network operators. Accordingly, the need for customization necessitates the digital twin model control in VL~6.             

In the conceptual virtualization architecture, VL~1 to VL~3 interface with the local controllers in the network, VL~4 and VL~5 interface with the centralized controller of the network, and VL~6 interfaces with both the local controllers and the centralized controller. This architecture fully exploits the two benefits of digital twins, i.e., providing extensive data for network management and enabling powerful network emulations. It also satisfies the aforementioned requirements for digital twins in terms of flexibility, compatibility, and customization. Last but not least, it answers the key questions regarding the implementation of digital twins raised in Subsection~\ref{ss:EUVirtual}.      

With the architecture design in Fig.~\ref{fig:digital_twin}, digital twins and network slicing are integrated in the idea of holistic network virtualization. Network slicing incorporates existing network virtualization techniques such as NFV. Digital twins enhance network slicing by providing organized and customized end user data to slices and by further abstracting slices into level-two digital twins. The design of two-level digital twins avoids extra resource consumption from creating and maintaining multiple digital twins of the same user for different slices and the resulting burden of synchronizing them. Instead, each slice has access to a subset of data from level-one digital twins pertinent to either the corresponding service or general user information such as location and mobility, and the pertinent data are further aggregated to the level-two digital twins for that slice. In this architecture, network slicing conforms to service-centric network management, while digital twins add a user-centric perspective to the virtualization. Specifically, level-one digital twins characterize end users and their service demands, and level-two digital twins  characterize network service provision capability, network performance, and network resource utilization. Overall, the digital twin paradigm and network slicing jointly support network management and service provision, while the network configures digital twins and network slices as needed, depending on network dynamics. %With such design, holistic network virtualization can empower 6G with unprecedented architectural flexibility, scalability, and adaptivity.         

%To further advance the network architecture design for 6G, processing   

%the digital twins contain selected data representing selected users for various services, while the content, accuracy, and synchronization frequency of the data are customizable. For example, despite of their benefits, introducing digital twins of all end users would consume extensive communication, storage, and computing resources. Therefore, the possibility of creating digital twins for selected end users is important. In the proposed architecture, Layer~6 can interact with Layer~5 to decide the criteria for selecting end users so that level-one digital twins are created only for these selected users.

% 

%With the above architecture for holistic network virtualization, digital twins and network slices are integrated under a unified network management framework. 

%In this architecture, the level-one digital twin of an end user is not a part of any specific slice but provides data for all slices involving that user. Each slice only has access to a subset of data in a digital twin, which is either pertinent to the service or general user information such as location and mobility. This avoids redundant resource consumption from creating and maintaining a digital twin of the same user in every slice and the burden of synchronizing these digital twins. The slice-specific access at level-one digital twins and slice-level processing with level-two digital twins facilitate service-oriented network management, which is aligned with the objective of network slicing. In the above architecture, level-one digital twins focus on characterizing end users and their service demands, while level-two digital twins and network slices focus on characterizing the service provision capacity, network performance, and network resource utilization.   


%Last but not least, both level-one and level-two digital twin models can be adjusted by Layer 6 as needed. The above properties guarantee the satisfaction of the aforementioned requirements on flexibility, compatibility, and customization. 




%what data goes into digital twin? Multiple use (for either service or management)
%delay justification


\subsection{Holistic Network Virtualization: A Summary}

In this section, we have reviewed the existing scope and techniques of network virtualization, identified the insufficiency of current network virtualization, introduced the idea of holistic network virtualization to incorporate network and end user virtualization, and developed a six-layer virtualization architecture for holistic network virtualization.  

The virtualization of resources, network functions, and networks in 5G is expected to remain important in 6G, since they contribute to flexible and adaptive network management. Meanwhile, the virtualization techniques in 5G, represented by network slicing and NFV, 
mostly focus on network virtualization from the perspective of service provision. In 6G, it will be essential to extend the scope of virtualization and incorporate end user virtualization. 

The digital twin paradigm is a promising solution to end-user virtualization. In 6G, digital twins can be used for characterizing the status and the service demand of individual end users. The study of digital twins in the context of 6G networks is still in an initial stage, and various definitions or implementations exist. In our vision of holistic network virtualization, digital twins are configurable assemblage of data, including both historical and real-time data and both collected and generated data, for describing end users, infrastructure, or network slices. Moreover, the corresponding data collection and processing are also configurable.   

To consolidate holistic network virtualization, we have proposed a six-layer virtualization architecture for 6G. The architecture provides a reference design for systematically integrating digital twins and network slicing and answers important questions related to digital twins in 6G networks, including where are they hosted, what data do they contain, and how to manage them.  

==> Final version/sec_Pervasive_Intelligence.tex <==



%In addition to holistic network virtualization, 




%In addition to holistic network virtualization, 

Pervasive network intelligence is the second element of our vision for 6G. In this section, we first present an overview of existing AI techniques. Then, we introduce the motivation and propose a four-level architecture for pervasive network intelligence. Next, we elaborate the idea of pervasive network intelligence from the perspectives of AI for networking and networking for AI, and review related works. Rather than surveying specific AI techniques, this section focuses on the architecture and methods of pervasive network intelligence. 

\subsection{{AI Techniques: An Overview}}\label{ss:AIOv}
\iffalse
 \begin{figure*}[tt]
	\centering
	\renewcommand{\figurename}{Fig.}
	\includegraphics[width=0.7\textwidth]{Fig/AI.pdf}
	%	\vspace{0cm}
	\caption{Some key ML algorithms.}
	\label{fig:digital_twin}
\end{figure*}
\fi
\begin{table*}[]
\caption{{Common ML algorithms.}}\label{table:AI}
\centering {
\begin{tabular}{|l|l|l|l|}
\hline
& Unsupervised Learning   & Supervised Learning   & Reinforcement Learning  \\ \hline
\begin{tabular}[c]{@{}l@{}}Centralized \\ Learning \\ Algorithms\end{tabular} & 
\begin{tabular}[c]{@{}l@{}} $\bullet$ K-means \cite{hartigan1979algorithm, Parwez}\\ $\bullet$ Mixture models \cite{topchy2004mixture,Shih}\\ $\bullet$ Autoencoders \cite{Bega}\\ $\bullet$ Generative adversarial\\ network \cite{ledig2017photo,Erpek} \end{tabular} &
\begin{tabular}[c]{@{}l@{}}$\bullet$ Support-vector machine \cite{SVM_MAC}\\ $\bullet$ Logistic regression \cite{You_LR}
\\ $\bullet$ Deep neural network \\ \cite{Peng_CNN,zhao2017lstm,Bega}\end{tabular} &
\begin{tabular}[c]{@{}l@{}}$\bullet$ Deep Q-learning \cite{DQN2,DQN1,Yaohua}\\ $\bullet$ Policy gradient\cite{silver2014deterministic,Somuyiwa,Hoang}\\ $\bullet$ Actor-critic \cite{konda2000actor,Cheng_AC}\\ $\bullet$ Deep deterministic policy \\gradient (DDPG) \cite{lillicrap2015continuous,TCCN_MUSHU,J_WWu2020}\end{tabular} \\ \hline
\begin{tabular}[c]{@{}l@{}}Distributed \\ Learning \\ Algorithms\end{tabular} & 
\multicolumn{2}{l|}{\begin{tabular}[c]{@{}l@{}}$\bullet$ Federated learning\cite{konevcny2016federated,Zhaohui}\\ $\bullet$ Split learning\cite{thapa2020advancements}\end{tabular}}                                                                                           
& \begin{tabular}[c]{@{}l@{}} $\bullet$ Multi-agent reinforcement learning\\ \cite{Weisen,Sana,Ruijin,Yunting}       \end{tabular}                                                                                                      \\ \hline
\end{tabular}}
\end{table*}
{The idea of AI is to design intelligent machines or systems to demonstrate human intelligence and perform tasks as humans do or even better~\cite{zhou2019edge}. The  advancement of machine learning (ML) has facilitated the success of AI in both academia and industry. Applications supported by ML techniques, such as computer vision and natural language processing, can achieve beyond human-level accuracy. Lately, for its potential in enabling intelligent networks, AI has received significant attention in the research field of wireless networks. }

{ML techniques can be categorized into three types: unsupervised learning, supervised learning, and reinforcement learning. In terms of learning structures, the techniques can be subdivided into centralized and decentralized techniques. We list common ML techniques used in wireless networks in Table \ref{table:AI}. }

{Unsupervised learning evaluates features and patterns hidden in data for data analysis, such as prediction, without using a labeled dataset. One popular application of unsupervised learning techniques is data clustering, e.g., \textit{k}-means \cite{hartigan1979algorithm} and mixture models \cite{topchy2004mixture}, for solving network planning problems, such as cluster-forming in wireless sensor networks \cite{Parwez} and small-cell deployment \cite{Samarakoon}. Neural networks can be adopted to facilitate novel unsupervised learning algorithms. For example, neural network-based autoencoders can learn the compressed features of input data with a limited number of neurons and can be leveraged for data prediction, such as traffic forecasting \cite{Bega}.}

{Supervised learning exploits the mapping between the input and output data via a given labeled dataset. Supervised learning techniques can derive a mapping function, i.e., a training model, from the input data to the labeled output data in the dataset. Through applying a training model, the output corresponding to a new input can be evaluated, which can be utilized for decision making or prediction. A typical method for supervised learning is using deep neural networks (DNNs). DNNs use layers of artificial neurons to estimate a non-linear correlation between the input and the output data and iteratively improve the estimation accuracy. There have been many successful applications of DNN techniques in communications. For example, convolutional neural networks (CNNs) utilize convolutional and pooling layers to identify the correlation of multi-dimensional input data and have been applied in modulation classification \cite{Peng_CNN}; recurrent neural networks (RNNs) explore the correlation among a sequence of the data and have been widely adopted for traffic prediction \cite{zhao2017lstm} and wireless channel modeling \cite{Zhu_RNN}.}

{Reinforcement learning iteratively learns the optimal policy by interacting with the environment, sensing network states, and evaluating feedback. The goal is to maximize a cumulative reward in a dynamic environment. 
Deep reinforcement learning (DRL), which combines DNN and reinforcement learning techniques, is used extensively in resource management to solve complex decision-making problems.
In DRL, neural networks play the role of approximators to store high-dimensional states or actions, which enables DRL to solve complex problems efficiently. DRL has been widely used for network optimization \cite{Yang_INFOCOM}, resource allocation \cite{J_WWu2020,DRL4,Somuyiwa}, and user association \cite{Cheng_AC,TCCN_MUSHU,Yaohua} in wireless networks.}

{With the development of mobile edge computing, distributed AI has been developed to harvest computing resources at network edge and reduce communication overhead due to data collection and exchange \cite{MEC_survey}. The learning models can be trained and evaluated at network edge in a semi- or fully-distributed manner. Specifically, federated learning (FL), as one of the most popular distributed learning techniques, trains models with data distributed over network edge. A centralized controller aggregates locally-computed learning models and updates parameters in the learning models.  Due to such decentralized model training, FL is capable of preserving privacy and can be applied in privacy-sensitive network management scenarios \cite{Niknam,lim2020federated}. In addition, multi-agent reinforcement learning has been developed to implement reinforcement learning in a distributed manner, which aims to handle scenarios in which network agents cannot obtain sufficient information from each other. Multi-agent reinforcement learning techniques can be used, for example, to solve resource allocation problems in heterogeneous networks \cite{Ruijin,Yunting}.  }


\subsection{Motivation and AI Architecture}\label{ss:Moti}
% \subsubsection{Motivation}\label{subsec:motivation}
In 6G, AI is expected to penetrate every facet of the network including end users, the network edge, and the cloud, resulting in \emph{pervasive network intelligence}. Such trend is due to advancements and innovations in the areas of ML, data collection, edge and cloud computing, and programmable network control in recent decades. As such, AI will fundamentally transform modern networks in many aspects and foster a myriad of exciting applications. 

% Fuelled by powerful computing facilities and well-curated datasets, AI techniques, especially deep learning (DL), can surpass traditional methods in a wide range of exciting applications from object detection and classification, audio recognition and content recommendation~\cite{gunduz2019machine, chen2019deep}. For instance, the learning based YOLO algorithm detects objects with a high accuracy, which can be applied in autonomous driving and mobile augmented reality applications~\cite{lin2018architectural,liu2018edge}. The state-of-the-art DL-based face recognition algorithm achieves an accuracy of more than 99\%~\cite{huang2008labeled}. These AI applications and many other future applications are expected to materialize in future 6G. In the presence of various R\&D initiatives on AI for telecommunications, AI applications in networks will flourish with innovative solutions. 

% why we have the idea of pervasive network intelligence



The AI applications can be categorized into management-oriented and service-oriented  applications, which are detailed as follows:
\begin{itemize}
	\item \emph{Management-Oriented AI Applications} - In these applications, AI is used as a tool for network management, such as transmission power allocation in cellular networks~\cite{sun2018learning} and resource reservation in network slices~\cite{J_WWu2020}. AI techniques, such as reinforcement learning, have the potential of handling complicated decision making problems in a dynamic network environment. Resorting to AI techniques, the management-oriented AI applications can analyze a large amount of network data, make real-time network management decisions, and then update network management policies based on the newly analyzed data. Hence, for such applications, the key issue is how to leverage advanced AI techniques to manage and enhance complex networks, which falls into the scope of \emph{AI for networking};
	
	\item \emph{Service-Oriented AI Applications} - In these applications, AI is offered as services for end users. Fuelled by powerful computing servers and well-curated datasets, AI techniques, especially  DL, can outperform traditional techniques in a wide range of applications, such as environmental perception in autonomous driving, audio recognition in intelligent healthcare, and object detection in mobile virtual reality~\cite{zhu2017overview, gunduz2019machine, chen2019deep}. For instance, an AI-based YOLO algorithm can detect objects with a high accuracy~\cite{lin2018architectural,liu2018edge}, and the state-of-the-art DL-based face recognition algorithm can achieve an accuracy of  99\% or higher~\cite{huang2008labeled}. Facilitating service-oriented AI applications in a network consumes a large amount of network resources, including storage  and computing resources for model training/inference, and communication resources for data collection and model uploading. Hence, for such applications, the key issue is how to design and optimize the network to support emerging AI services, which falls into the scope of \emph{networking for AI}. 
\end{itemize}
Note that the scope of AI in 6G includes AI for networking and networking for AI, which is larger than that in 5G, as the latter simply focuses on  applying AI in  communications.


%, while data aggregation and management problems are emerged. 
% As the results, it is critical to efficiently allocate the resources within a RAN for the applications, especially for the edge AI case.


\begin{figure}[t]  
	\centering  
	\includegraphics[width=92mm]{Fig/fig2.pdf}\\
	\caption{An illustration of the four-level AI architecture for pervasive network intelligence.}  
	\label{fig:1} 
\end{figure}



% \subsubsection{Four-Level AI Architecture}\label{subsec:layered_architecture}
An AI architecture is needed to characterize AI's different functionalities in different network segments. In the literature, there are a few studies on the AI architecture. Edge intelligence (or edge AI) is represented in six levels based on the amount and path length of data offloading~\cite{zhou2019edge}. Moreover, edge intelligence can be categorized into two parts: AI for edge (i.e., to enhance and optimize the network edge with AI techniques) and AI on edge (i.e., to carry out AI models on the network edge)~\cite{deng2020edge, peltonen20206g}. Different from these works on edge intelligence, our work focuses on a broader scope of pervasive network intelligence and categorizes it into multiple levels based on AI's locations and functionalities in the network. 


%For different AI applications in 6G networks, AI can reside at different locations in the network. Hence, 
As shown in Fig.~\ref{fig:1}, we propose a four-level AI architecture, in which AI levels (ALs)~1 and 2 focus on service-oriented applications, and ALs~3 and 4 aim at management-oriented applications. We describe each level in detail as follows.
%\begin{itemize}

\emph{AL 1 - End User-Hosted Service-Oriented AI}: Utilizing local data and computing resources at end users, end user-hosted service-oriented AI applications are offered as services for end users by processing AI tasks locally, such as next word prediction in mobile keyboards~\cite{hard2018federated}, user traffic demand prediction~\cite{wang2020cellular}, and vehicle trajectory prediction~\cite{deo2018convolutional}. When computing resources of end users are insufficient for computation-intensive AI tasks, partial computation workloads can be offloaded to nearby edge servers for collaborative processing.  

\emph{AL 2 - Edge-Hosted Service-Oriented AI}: Residing at network edge (e.g., Wi-Fi access points and BSs) close to end users, edge-hosted service-oriented AI applications are offered as low-latency services for end users, such as face recognition in video surveillance~\cite{cocskun2017face} and object detection in virtual reality~\cite{erhan2014scalable}. To support edge-hosted service-oriented AI applications, service demand data from end users are collected, stored, and analyzed, and then the analytical results are utilized for service provision.   
	
	% Edge-hosted AI applications need the collaboration among the edge servers to facilitate services. In addition to collecting data from device-hosted AI on end users, edge-hosted AI needs to collect more information, such as historical service data and previous deployed AI models. 
	
\emph{AL 3 - {Edge-Hosted} Management-Oriented AI}: At this level, AI is hosted at local  controllers at  network edge for network management that is executed in real time, such as spectrum allocation, content caching~\cite{muller2016context}, and computation  offloading~\cite{zhou2020deep}. Specifically, the edge-hosted management-oriented AI is  to allocate network resources to network nodes for supporting services, including AI services at ALs~1 and~2. For instance, the edge-hosted management-oriented AI can be used to perform service migration across edge networks to guarantee service continuity for high-mobility users, e.g., vehicular users. %The required data of AI applications are aggregated user data, which are processed to find a network operation policy; 
	
\emph{AL 4 - Cloud-Hosted Management-Oriented AI}: Cloud-hosted management-oriented AI resides at the centralized controller in the cloud for network management that is executed once every several minutes or hours, such as slice admission control~\cite{sciancalepore2019rl} and virtual network function deployment~\cite{qu2020dynamic}. Since the cloud possesses abundant computing and storage resources, powerful and complex  AI models can be trained and deployed for managing large-scale networks.
	
%\end{itemize}
% Note that AI applications at higher levels cover more users. As a result, the raw data from end users should be aggregated and abstracted, such that AI applications at the higher levels can make decisions in a flexible and scalable manner.




Next, AI for networking is elaborated in Subsection~\ref{ss:AIforNet} to illustrate AI's role in network management, and networking for AI is discussed in Subsection~\ref{ss:NetforAI} to illustrate AI service provision in 6G networks.








\subsection{AI for Networking}\label{ss:AIforNet}

In this subsection, we discuss how AI techniques can support network management. We first review existing works on AI-based network slicing. Then, we introduce our idea of connected AI solution for AI-based network slicing.
%for network management, which aims to efficiently integrate AI-empowered network control modules in future networks.


\begin{table*}[h]
	\centering
\scriptsize{
	\caption{Representative Works on AI-based Network Slicing}\label{Table:NetworkSlicing}
\begin{tabularx}{0.92\textwidth}{|p{1.2cm}|l|p{3cm}|p{6cm}|X|} %0.97\textwidth last column p{3cm} for 1-column
\hline
\textbf{Stage}    &  \textbf{Work} & \textbf{Research Focus}  & \textbf{Objective}  &  \textbf{AI Method} \\ \hline
\multirow{13}{*}{{\shortstack[l]{Network\\Planning}}}  & \cite{Bega} & Network capacity prediction  & Forecasting the capacity for individual virtual networks & Deep neural network based autoencoder \\ \cline{2-5}
 & \cite{J_HWang2020} & Virtual representation for network slices & Capturing the relationships among slices and monitoring the end-to-end performance in dynamic network environments & Graph neural networks \\\cline{2-5}
 & \cite{Huynh} & Resource reservation adjustment &  Maximizing the overall reward obtained from the tenants of slices & Deep dueling neural networks \\\cline{2-5}
 & \cite{gnn2} &  Bandwidth allocation &  Jointly maximizing spectrum efficiency and the QoS requirement satisfaction ratio & Generative adversarial network and deep Q network\\\cline{2-5}
 & \cite{Li_CL}& Bandwidth allocation & Jointly maximizing spectrum efficiency and overall service level agreement satisfaction ratio of slices& Long short-term memory and advantage actor-critic\\\cline{2-5}
 & \cite{Chergui} & Traffic prediction and resource provisioning & Minimizing the probability of slice service level agreements violation & Gated recurrent unit\\
 \hline
\multirow{13}{*}{{\shortstack[l]{Network\\ Operation}}}  & \cite{drl2} & Computation offloading & Minimizing average computing time of services and maximizing user computing experience & Deep Q network\\ \cline{2-5}
& \cite{Xiang_TVT} & Slice selection and channel allocation & Minimizing the power consumption of wireless transmission for a sliced fog-RAN & Reinforcement learning \\ \cline{2-5}
& \cite{Xiang_TWC} & Content caching placement and delivery &  Managing caching resources to maximize cache hit ratio while satisifying resource reservation constraints & Deep Q network\\ \cline{2-5}
& \cite{Chen_JSAC} & Inter-slice coordination  & Maximizing long-term payoff from the competition among service providers through resource orchestration & Deep Q network\\ \cline{2-5}
& \cite{Messaoud}& Inter-slice coordination &  Maximizing QoS satisfaction ratio for slices by scheduling transmission power and sharing resources among slices & Multi-agent deep Q learning\\
\hline
\multirow{5.5}{*}{{\shortstack[l]{Two-Stage\\Interplay}}}  & \cite{J_WWu2020} & Computing resource allocation in vehicular networks & Allocating spectrum and computing resources for slices while minimizing computing service delay & Deep deterministic policy gradient  \\ \cline{2-5}
&\cite{Dandachi} &  Cross-slice admission and congestion control & Maximizing operator revenue by resource reservation and adjust reserved resources in real time & State-action-reward-state-action (SARSA) \\
\hline
\end{tabularx}
}
\end{table*}

%%%%%%%%%%%%%%------------------------------%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{AI-Based Network Slicing}\label{ss:AISlicing}


Network slicing includes two stages: network planning stage for resource reservation and network operation stage for resource scheduling~\cite{J_XShen_2020}. In the \textit{network planning} stage, network resources are reserved for network slices on a large time scale (e.g., from several minutes to several hours).  In the \textit{network operation} stage, the reserved resources of each slice are allocated to end users on a small time scale (e.g., from several milliseconds to several seconds). Due to network dynamics such as spatiotemporally changing network traffic, it can be difficult for model-based solutions to attain the optimal network slicing strategies. By contrast, AI techniques can characterize network dynamics by analyzing the collected network data and obtain the optimal network slicing strategies accordingly. Next, we review AI-based network slicing, taking into account the interplay between the planning and operation stages. Representative research works on AI-based network slicing are summarized in Table~\ref{Table:NetworkSlicing}.


%Effective AI-based network slicing depends on the availability and quality of data from the network, e.g., end user location and mobility.
%To efficiently collect and analyze real-time data, a local controller on network edge collects end user data from level one digital twin and AI applications deployed at the network edge, i.e., AL~1 and AL~2 applications. Specifically, the results from AI-based data analysis in AL~1 and AL~2 applications may provide additional user information for network management. For instance,  simultaneous localization and mapping (SLAM) technique for applications, such as localization in autonomous driving, determines user location based on images by Kalman filter~\cite{Chatterjee} or DNNs~\cite{zhang2017neural}~\cite{SLAM}, which requires intensive image processing at edge devices.

On a small time scale, a local controller collects data and provides resource scheduling strategies to allocate resources reserved for each slice to end users. Specifically, the local controller determines resource scheduling strategies based on two factors: the amount of resources reserved for each slice, which is determined by the centralized controller, and the instantaneous user data from level-one digital twins pertinent to that slice, such as service type, user location, and user mobility. The main challenges of determining the optimal resource scheduling strategies are two-fold: a large number of end users and service demand dynamics. AI techniques have potentials to cope with both challenges. First, to schedule resources for a large number of end users, unsupervised learning methods, such as \textit{k}-means~\cite{kmean} and DNN based autoencoders~\cite{Bega}, can be utilized to classify end users according to their service demands. Similar resource scheduling strategies can be applied to end users with similar service demands, which facilitates scalable network management. For instance, end users in close proximity and with similar mobility patterns may experience similar channel statistical behaviors, and the same power control policy can be applicable to them. Second, to deal with network dynamics, reinforcement learning can be applied for generating adaptive resource scheduling strategies~\cite{drl1}.  Reinforcement learning iteratively allocates resources to maximize a long-term reward function and updates the reward function based on feedback from the network environment. Moreover, reinforcement learning can be combined with DNNs, such as recurrent neural networks~\cite{J_MLi2021} and conventional neural networks~\cite{TCCN_MUSHU}, to analyze the spatiotemporal pattern of user data for finding the optimal resource scheduling strategies. %\textcolor{blue}{The above AI-driven approaches for network operation correspond to AL 3 in Fig.~\ref{fig:1}.}

On a large time scale, local controllers aggregate the collected user-level data to service-level information from level-two digital twins, i.e., slice digital twins. Utilizing information from slice digital twins, the centralized controller reserves network resources for each slice. The challenges of resource reservation are two-fold. First, making proactive resource reservation that can avoid either resource over-provisioning or under-provisioning is challenging with time-varying network traffic. Second, the strategies for resource reservation and scheduling are coupled, which further complicates resource reservation. AI techniques can cope with these challenges as follows. To address the challenge of proactive resource reservation, supervised learning, such as long short-term memory (LSTM) networks, can be used to exploit the features of historic network traffic loads and predict traffic loads in near future~\cite{Li_CL, wang2020cellular}. The centralized controller can then use the predicted traffic loads for proactive resource reservation.
To handle the correlation between resource reservation and scheduling, reinforcement learning can be adopted to reserve resources while considering network operation strategies as a part of the  dynamic network environment~\cite{J_WWu2020,DRL4, Chen_JSAC}. Moreover, an option-based hierarchical reinforcement learning technique can be a potential solution for jointly optimizing resource reservation and network operation policies and addressing network dynamics in both stages. This technique has been used to tackle complex DRL problems by grouping decision variables according to decision time scales~\cite{HDL1} or decision-making agents~\cite{Qian} and then determining the decision variables. Through this novel reinforcement learning technique, the complex correlation between resource reservation and scheduling strategies can be obtained iteratively. To apply this technique in network slicing, the centralized controller can select the resource reservation strategies on a large time scale, and local controllers find optimal resource scheduling strategies on a small time scale, thereby jointly optimizing both the resource reservation and the scheduling strategies. %\textcolor{blue}{The AI applications for network planning correspond to AL 4 applications in Fig. \ref{fig:1}.}





\subsubsection{Connected AI Solution for Network Management}\label{ss:nested}
%integration
Existing AI applications on network management mostly focus on individual control functions.
For instance, learning-based autoencoders can achieve reliable transmission power control for high-speed data transmission with limited channel state information~\cite{Dorner}, and DNNs can select medium access control protocol parameters with low communication and processing overhead~\cite{JieG_mac1},\cite{Jie_mac2}. 
Although various AI techniques have been proposed for network management, AI models among network control functions are usually isolated. Such isolation may result in inefficient and redundant data processing, which brings up a pressing need for integrating the AI models in AI-based network control functions. 
% To support various network control functions as a whole, an integrated AI model is required. 


There are three types of solutions for integrating AI models~\cite{M_ZZhang_2019}. In the first type of solutions, the entire network is viewed as a black box, where a single AI model characterizes the entire network and generates network control policies. Such structure simplifies decision-making processes in network management. However, training the single AI model can be extremely difficult due to high-dimensional input data. Then, the second type of solutions adopts different AI models in a network for different network control functions, and the AI models are generally independent on each other to reduce the complexity of training. However, this approach neglects the correlation and interplay among network functions and thus cannot obtain a global-optimal network management strategy. Moreover, network data may be repetitively processed by different AI models with similar network functions, which degrades network management efficiency. For instance, AI models for user mobility management and computing service migration would repetitively analyze end user mobility. In contrast, the third type of solutions, namely \textit{connected AI}, exploits the correlations among network control functions, connects their AI models, and allows them to jointly make network control decisions. The connected AI solution offers benefits in integrating AI models by highlighting the interplay among them and balancing training complexity and network performance. Therefore, the connected AI solution has great potential in facilitating AI-based network slicing. However, existing research on the connected AI solution is limited. How to apply connected AI solution to network management requires further studies~\cite{M_SHan2020}.

Recent advancements in distributed learning techniques facilitate the development of a connected AI solution for network management. Model partition, investigated in~\cite{Yiping}, can divide a global DNN into multiple sub-neural networks (sub-NNs). The sub-NNs can reside at different network entities, according to the available computing and communication resources, and communicate with each other~\cite{partition1, partition3}. Furthermore, the idea of \textit{nested DNN}, which allows sub-NNs to have their own functionalities while contributing to the global DNN for model inference and training, has been proposed and evaluated in~\cite{cui2021fully} and~\cite{nest1}. Using the above two techniques, each sub-NN can perform a specific network control function. Accordingly, multiple sub-NNs can collaboratively fulfill common control functions, thereby applying the connected AI solution to network management.


\begin{figure}[t]  
  \centering  
%   \includegraphics[width=90mm]{Fig/ai_for_slice2_new}\\
    \includegraphics[width=90mm]{Fig/fig3-new.pdf}\\
  \caption{The connected AI solution for network management.}  
  \label{fig:3} 
\end{figure}

Based on the above advanced DNN techniques, we present our idea of applying the connected AI solution to network management next. The control functions for network management are encapsulated into \textit{intelligent modules}. An intelligent module can be implemented solely by a DNN or cooperatively by a DNN and conventional model-based techniques. An example is shown in the upper right corner of Fig.~\ref{fig:3}, in which the intelligent module for power control includes a learning-based channel estimator and a model-based power allocation scheme, e.g., water-filling power allocation~\cite{Haykin}. Moreover, the DNN in each intelligent module can play the role of a sub-NN of a global DNN. 
The intelligent modules connect with each other to share information, such as their outputs and gradient information in model training, and aggregated user data.
Via the intelligent modules, control functions can manage the network in a divide-and-conquer manner to avoid the complicated model training required for layer-free AI. With model partition and nested DNN techniques, multiple network control functions can cooperatively make control decisions to achieve globally optimal network management.

Fig.~\ref{fig:3} shows another example of the connected AI design, i.e., supporting mobile edge computing. We explain the design using the case of  vehicular networks as an example. Note that other networks can use the same or a similar design. Small base stations (SBSs), as edge servers, can process computation tasks offloaded by vehicles. Intelligence modules at SBSs provide computing offloading decisions, including the computing tasks to be offloaded, transmit power for offloading, task scheduling, etc., based on network status and computing offloading requests. Due to the high mobility of vehicles and the limited communication coverage of the SBSs, computing tasks are often migrated among the SBSs, referred to as service migration, and migration decisions are determined by a macro base station (MBS). Service migration and computing offloading decisions are highly coupled. For example, the chance of service migration increases when  vehicles offload more computing tasks to an SBS. In addition, service migration requires the collaboration of multiple SBSs. In our idea of connected AI, service migration and computing offloading decisions are jointly determined. Specifically, we split the DNN into multiple sub-NNs by DNN splitting and nested DNN techniques. Some sub-NNs are deployed at the SBSs to provide computing offloading decisions.  These sub-NNs are also connected with a sub-NN deployed at an MBS, which can be leveraged to make migration decisions. In this example, the input of the service migration module includes the output of intelligent modules at the SBSs, e.g., computing offloading decisions and the parameters of sub-NNs, and the output of the service migration module is the service migration policy. In this way, the intelligent modules can cooperate to make decisions for mobile edge computing.













%%%%%%%%%%%%%%------------------------------%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%------------------------------%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\subsection{Networking for AI}\label{ss:NetforAI}
%1. concept and motivation of networking for AI; 2. model training and model inference, existing works on model training and model inference; 3. challenges   


In addition to managing networks, AI can function as services, namely {AI services}, which reside at ALs~1 and~2 in the proposed AI architecture in Fig.~\ref{fig:1}. \emph{Networking for AI} is to design and optimize networks to facilitate AI services. In this subsection, we first introduce the motivation of networking for AI. Next, existing works are reviewed, and research challenges are presented. Finally, the idea of AI slice is proposed and elaborated. 
%In addition to managing networks , AI can be offered as services, which motivates people to think in the reverse perspective, i.e., networking for AI. 






%Then, we propose two designs, i.e., AI instance and AI slice, to support AI services in  networks.

\subsubsection{Motivation}\label{subsubsec: Motivation}
%With the great potential of AI in managing networks (i.e., AI for networking), a new research area on how to facilitate AI services in future networks has emerged, referred to as \emph{networking for AI}. 
Networking for AI is attracting great attention in both academia and industry. In academia, networking for AI calls for extensive interdisciplinary research efforts between networking researchers and AI researchers to develop new communication standards and technologies to cater for  AI services at scale~\cite{chemouil2019special, sorour2020returning, gunduz2019machine,wu2021ai}. In industry, the International Telecommunication Union (ITU) is discussing high-level architectures to integrate, orchestrate, and update AI components for future networks, including IMT-2020 networks~\cite{itu2019architectural, itu2019Unified}. Some 3GPP working groups are studying data collection frameworks in the network for supporting AI services~\cite{3GPP2019Study, wilhelmi2020flexible}. Notably, networking for AI is becoming an indispensable component for facilitating AI services in networks and is expected to be a key enabling technology in 6G. 



%According to the location where a model is trained, the training manner can be categorized into: (i) centralized training that trains the model in one node, e.g., cloud model training, in which all data is collected and uploaded to a cloud server for model training; and (ii) decentralized training that trains the model at multiple nodes in a distributed manner, e.g., federated learning~\cite{hard2018federated, li2020federated}, in which end users cooperate to train a global  model with local data under the coordination of an edge or cloud server. Decentralized training can reduce communication resource consumption and preserve data privacy, since the data is processed locally. Note that AI models should be periodically retrained based on fresh data in a changing environment; otherwise, well-trained models can be outdated, rendering significant inference performance degradation. 
%As mentioned, AI will be pervasive in 6G networks, and every network nodes is equipped with build-in AI capability. 

Networking for AI should take the following factors into consideration:
\begin{itemize}
    \item \emph{Distributed Data} -  With the wide deployment of various IoT devices and small BSs, massive data are generated from many distributed network nodes, e.g., end users and the network edge. In the traditional cloud-based AI paradigm, the cloud  collects massive distributed data for model training, and a well-trained model is deployed at the cloud for model inference. This paradigm suffers from spectrum resource scarcity and user privacy leakage concerns.\footnote{Google's autonomous driving vehicle can generate more than 750\;MB of data per second~\cite{va2016millimeter}.} To address these issues, a potential solution is to facilitate AI services over a large number of network nodes in a distributed manner~\cite{hard2018federated}, which requires new networking protocols to coordinate multiple network nodes;
    
    \item \emph{Constrained Resources} - Network nodes, such as end users, have limited resources, while state-of-the-art AI models (e.g., DNN models with dozens of neural network layers) are complex. As such, running a complex AI model on a single network node can exhaust its computing resource and energy.\footnote{The energy consumption of using AlexNet to process an image on a tailored energy-efficient Eyeriss chip is up to 0.28\;W~\cite{chen2016eyeriss}.} With advanced model partition techniques (e.g., DNN partition), a complex AI model can be partitioned into multiple sub-models and embedded into a network with data exchange among the sub-models~\cite{model_partition}. Executing sub-models consumes computing resources of network nodes, and exchanging data between sub-models also consumes communication resources. Hence, running AI models at multiple network nodes in a cost-effective manner requires innovative network embedding designs;
    
    \item \emph{Network Heterogeneity and Dynamics} - 6G networks will be highly heterogeneous, in which network nodes possess different amounts of communication, computing, and storage resources. As complex AI models need to be deployed at multiple network nodes, executing AI tasks requires judiciously allocating resources of these network nodes. Moreover, network dynamics, such as time-varying channel conditions among network nodes and spatiotemporal service demands, further complicate the resource allocation decision making problem. Hence, it is necessary to design tailored resource management algorithms to optimize AI performance, while adapting to network dynamics.
\end{itemize}
% {Overall, the factors pose challenges on facilitating AI services in the network,} thereby calling for new designs in networking protocols, network embedding, and resource management.


%Taking the above factors into account, implementing efficient AI requires fundamental changes in and innovative designs of wireless networking protocols. 

%\subsubsection{Network Architecture and Performance Metrics}


%\subsubsection{}
%Beyond traditional computation services, AI services focus on multi-dimensional performance metrics: communication cost, latency, energy consumption, etc. Different stages focus on different performance metrics.
The \emph{scope} of networking for AI covers the entire lifecycle of AI services, which consists of three stages. The first stage is \emph{data collection} for model training via  communication links. For instance, real-time service load data from end users need to be collected to train an AI model for service demand prediction. The second stage is \emph{model training}, which is to achieve a certain objective based on the collected data. For instance, a large number of images are processed to train DNN-based object detection modules until  the target accuracy requirement is satisfied. The third stage is \emph{model inference}, which is to apply well-trained models to complete specific computation tasks. For instance, AI-based object recognition for autonomous driving detects and classifies nearby vehicles, pedestrians, and obstacles based on real-time images captured by on-board cameras~\cite{lin2018architectural}. %All the three stages impact the performance of AI services. %To optimize AI service performance, tailored designs in different networks for all the three stages are required.

% Existing networking protocols and resource management schemes data-centric
% Hence, 


\subsubsection{State-of-the-Art Approaches}\label{subsubsec: related_work}
%Unlike AI for networking area, which has abundant research works, only a few research works devote to networking for AI area. However, networking for AI is becoming a hot research topic since a significant increase in publications in this area. 
The research on networking for AI is still at its infancy stage with only a few existing works. In this subsection, the existing studies are categorized into data collection, model training, and model inference according to the lifecycle of AI services. Representative related works are summarized in Table~\ref{Table:networking_for_AI}.

\begin{table*}
	\centering
	\scriptsize{
		\caption{Summary of Related Works on Networking for AI} \label{Table:networking_for_AI}
% 		\begin{tabularx}{0.85\linewidth}{|>{\hsize=0.15\hsize}X|>{\hsize=0.1\hsize}X|>{\hsize=1.3\hsize}X|>{\hsize=0.4\hsize}X|} 
		\begin{tabularx}{0.92\textwidth}{|l|l|p{10cm}|X|}
		%1st column 0.25, second column 0.14, third column 2, last column 0.6 for 1 column mode
			\hline
			\textbf{Topic}  & \begin{tabular}[c]{@{}l@{}} \textbf{Work}\end{tabular}  & \textbf{Contribution} & \textbf{Highlight}     \\ \hline
			\multirow{5}{*}{\begin{tabular}[c]{@{}l@{}} Data \\Collection \end{tabular}}  
			&\centering \makebox{ \cite{wen2019overview}}  
			&  Scheduling data transmission based on users' data importance levels and channel conditions           &  Data importance-aware spectrum allocation  \\ \cline{2-4} 
			&\centering \makebox{\cite{wang2020machine}}  &  Allocating users' transmission power that can adjust the amount of  collected data  samples for multiple AI models to enhance the overall model accuracy    & Data amount-aware power allocation  \\ \cline{2-4} 
			&\centering \makebox{\cite{liu2020wireless}}  &  Designing an importance-aware ARQ  protocol, in which users' data importance levels and channel conditions are jointly considered to trigger data retransmission   &  Data importance-aware  retransmission protocol  \\ \hline
			
			\multirow{11}{*}{\begin{tabular}[c]{@{}l@{}}Model\\ Training\end{tabular}} 
			&\centering \makebox{\cite{liu2020client}}  &  Proposing an edge-cloud assisted FL framework, in which the edge and cloud servers alternatively aggregate local models to reduce communication overhead  &  Two-tier FL framework     \\  \cline{2-4} 
			&\centering \makebox{\cite{yang2020federated}}  &  Proposing an over-the-air computation approach for model aggregation   &  Over-the-air model   aggregation  \\ \cline{2-4} 
			&\centering \makebox{\cite{wang2020optimizing}}  &  Selecting users with more contribution to  convergence for model aggregation based on users' data distribution  &  Data distribution-aware user selection    \\  \cline{2-4} 
			&\centering \makebox{\cite{nishio2019client}}  &  Selecting  users with low training delay considering heterogeneity among  users  & Training latency-aware user selection  \\  \cline{2-4} 
			&\centering \makebox{\cite{wang2019adaptive}}  &  Optimizing the number of local model updates given a  resource budget &  Local update frequency optimization   \\  \cline{2-4} 
			&\centering \makebox{\cite{ren2020scheduling}}  &  Scheduling model uploading based on end users' model importance levels and channel conditions    &   Model importance-aware  model uploading  \\\hline
			
				\multirow{8}{*}{\begin{tabular}[c]{@{}l@{}}Model\\ Inference\end{tabular}}  
			&\centering \makebox{\cite{liu2018edge}}  & Optimizing video frame rate and input image resolution to balance service latency and   detection accuracy for virtual reality users  &  Data resolution optimization  \\  \cline{2-4} 

			&\centering \makebox{\cite{wang2020joint}}  &  Selecting the optimal DNN model for real-time video analytics    &   DNN model selection  \\  \cline{2-4} 
			&\centering \makebox{\cite{zhang2021autodidactic}}  &  Selecting the optimal DNN model's cut layer  to minimize inference latency  for user-edge DNN synergy     &   User-edge DNN model partition  \\  \cline{2-4} 
			&\centering \makebox{\cite{teerapittayanon2017distributed}}  & Partitioning a complicated DNN model across end users, the network edge, and the  cloud to reduce communication overhead    &  User-edge-cloud DNN model partition \\ \cline{2-4} 
		    &\centering \makebox{\cite{wu2020accuracy}}  & Designing a collaborative DNN model inference scheme with light-weight models at IoT devices and an uncompressed model at the network edge   & Collaborative DNN model inference \\  \cline{2-4} \hline

	\end{tabularx}}
\end{table*}


% \begin{table*}
% 	\centering
% 	\scriptsize{
% 		\caption{Summary of Related Works on Networking for AI} \label{Table:networking_for_AI}
% 		\begin{tabularx}{0.85\linewidth}{|>{\hsize=0.2\hsize}X|>{\hsize=0.1\hsize}X|>{\hsize=1.3\hsize}X|>{\hsize=0.4\hsize}X|} %1st column 0.25, second column 0.14, third column 2, last column 0.6 for 1 column mode
% 			\hline
% 			\textbf{Topic} & \begin{tabular}[c]{@{}l@{}} \textbf{Work}\end{tabular}  & \textbf{Contribution} & \textbf{Highlight}     \\ \hline
% 			\multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}Data\\ Collection\end{tabular}}  
% 			&\centering \makebox{ \cite{wen2019overview}}  & \begin{tabular}[c]{@{}l@{}} Schedule data transmission based on users' data importance levels and channel \\conditions  \end{tabular}         & \begin{tabular}[c]{@{}l@{}} Data importance-aware \\spectrum allocation     \end{tabular}                                   \\ \cline{2-4} 
% 			&\centering \makebox{\cite{wang2020machine}}  & \begin{tabular}[c]{@{}l@{}} Allocate users' transmission power that can adjust the amount of  collected data \\ samples of multiple AI models to enhance the overall model accuracy  \end{tabular}  & \begin{tabular}[c]{@{}l@{}} Data amount-aware \\power allocation \end{tabular} \\ \cline{2-4} 
% 			&\centering \makebox{\cite{liu2020wireless}}  & \begin{tabular}[c]{@{}l@{}} Design an importance-aware ARQ  protocol, in which users' data importance levels \\and channel conditions are jointly considered to trigger data retransmission \end{tabular}  & \begin{tabular}[c]{@{}l@{}} Data importance-aware \\ retransmission protocol \end{tabular} \\ \hline
			
% 			\multirow{11}{*}{\begin{tabular}[c]{@{}l@{}}Model\\ Training\end{tabular}} 
% 			&\centering \makebox{\cite{liu2020client}}  & \begin{tabular}[c]{@{}l@{}} Propose an edge-cloud assisted FL framework, in which the edge and cloud servers\\ alternatively aggregate local models to reduce communication overhead \end{tabular} & \begin{tabular}[c]{@{}l@{}} Two-tier model\\ aggregation  \end{tabular}  \\  \cline{2-4} 
% 			&\centering \makebox{\cite{yang2020federated}}  & \begin{tabular}[c]{@{}l@{}} Propose an over-the-air computation approach for model aggregation \end{tabular}  & \begin{tabular}[c]{@{}l@{}} Over-the-air model \\  aggregation \end{tabular} \\ \cline{2-4} 
% 			&\centering \makebox{\cite{wang2020optimizing}}  & \begin{tabular}[c]{@{}l@{}} Select end users with more contribution to  convergence for model aggregation \\based on end users' data distribution \end{tabular} & \begin{tabular}[c]{@{}l@{}}Data distribution-aware\\ end user selection  \end{tabular} \\  \cline{2-4} 
% 			&\centering \makebox{\cite{nishio2019client}}  & \begin{tabular}[c]{@{}l@{}} Select end users with low training delay considering heterogeneity among end users  \end{tabular}& \begin{tabular}[c]{@{}l@{}}Delay-aware end \\user selection  \end{tabular}\\  \cline{2-4} 
% 			&\centering \makebox{\cite{wang2019adaptive}}  & \begin{tabular}[c]{@{}l@{}}  Optimize the number of local model updates given a  resource budget \end{tabular} & \begin{tabular}[c]{@{}l@{}} Local update frequency\\ optimization  \end{tabular} \\  \cline{2-4} 
% 			&\centering \makebox{\cite{ren2020scheduling}}  & \begin{tabular}[c]{@{}l@{}} Schedule model uploading based on end users' model importance levels and \\  channel conditions   \end{tabular} &  \begin{tabular}[c]{@{}l@{}} Model importance-aware \\ model uploading  \end{tabular}\\\hline
			
% 				\multirow{8}{*}{\begin{tabular}[c]{@{}l@{}}Model\\ Inference\end{tabular}}  
% 			&\centering \makebox{\cite{liu2018edge}}  & \begin{tabular}[c]{@{}l@{}}Optimize video frame rate and input image resolution to balance service latency and \\  detection accuracy for virtual reality users \end{tabular} & \begin{tabular}[c]{@{}l@{}} Data resolution\\ optimization  \end{tabular}\\  \cline{2-4} 
% 			&\centering \makebox{\cite{wu2020accuracy}}  & \begin{tabular}[c]{@{}l@{}}Design an adaptive sampling rate configuration scheme according to channel \\conditions for DNN-based fault diagnose services in industrial IoT networks \end{tabular} & \begin{tabular}[c]{@{}l@{}} Sampling rate\\ adaption \end{tabular}\\  \cline{2-4} 
% 			&\centering \makebox{\cite{wang2020joint}}  & \begin{tabular}[c]{@{}l@{}} Select the optimal DNN model for real-time video analytics   \end{tabular} &  \begin{tabular}[c]{@{}l@{}} DNN model selection \end{tabular} \\  \cline{2-4} 
% 			&\centering \makebox{\cite{zhang2021autodidactic}}  & \begin{tabular}[c]{@{}l@{}} Select the optimal DNN model cut layer  to minimize inference latency  \\ for user-edge DNN synergy     \end{tabular} &  \begin{tabular}[c]{@{}l@{}} DNN cut layer\\ selection \end{tabular}\\  \cline{2-4} 
% 			&\centering \makebox{\cite{teerapittayanon2017distributed}}  & \begin{tabular}[c]{@{}l@{}} Partition a complicated DNN model across end users, the network edge, and the  \\cloud to reduce communication overhead     \end{tabular} &  \begin{tabular}[c]{@{}l@{}} User-edge-cloud \\ model partition \end{tabular}\\ \hline

% 	\end{tabularx}}
% \end{table*}


\textbf{Data Collection} - The objective is to efficiently collect the data from end users for optimizing AI performance. Since data are distributed across end users in the network, transmission resource is scheduled to end users for uploading their data. For instance, the level-one digital twins require periodical data synchronization with the end users, and such data can be provided for AI services. Data collection is a classic research problem widely investigated in wireless sensor networks~\cite{li2017wireless} and UAV networks~\cite{zhan2017energy}, and these works focus on optimizing either the reliability of data collection or the amount of  collected data. {In AI services, the collected data are used to train AI models, and the data samples may have different importance levels for model training. Merely maximizing the reliability or the amount of the collected data is not optimal. Hence, novel data collection designs taking model training into account are required for performance optimization. }

%Hence, redesigning traditional data collection schemes is needed.

%The conflict between large amount of data and limited spectrum resource results in prohibitive data collection latency, which calls for efficient data collection schemes target at learning performance. Since more data contributes to a better model, traditional data collection schemes are to maximize the amount of uploaded data which mainly takes users' channel conditions into account, rather than optimizing learning performance.




Recently, AI-centric data collection is investigated in the following two research directions:
\begin{itemize}
    \item  \emph{Resource Allocation} -  Data importance-aware resource allocation schemes have been proposed to optimize AI model accuracy. The idea is to schedule data transmission while taking both end users' channel conditions and data importance levels into account~\cite{wen2019overview}. The data importance level can be captured via data uncertainty, i.e., higher uncertainty means higher importance. The data uncertainty can be measured by entropy~\cite{holub2008entropy}. {Power allocation for data collection is investigated in multi-model training scenarios~\cite{wang2020machine}. Since the number of  collected data samples impacts the model accuracy, a learning-centric power allocation scheme can adjust the users' transmission power to determine the amount of  collected data  for different AI models, thereby maximizing the overall model accuracy given a transmission power budget;}
    
    
    \item\emph{Protocols} - There are a few AI-centric data collection protocols. In a  network environment with poor channel conditions, data retransmission is applied to improve data collection reliability. Existing automatic repeat-request (ARQ) retransmission protocols, such as hybrid ARQ in long term evolution (LTE) networks, trigger data retransmissions for lost packets once the end user's signal-to-noise ratio (SNR) threshold is satisfied. The importance of data samples should be incorporated in transmission protocols to speed up the model training process. An importance-aware ARQ  protocol is proposed for CNN-based classification model training in~\cite{liu2020wireless}. In the protocol, both data importance levels and channel conditions are taken into account to determine the data retransmission threshold, which can enhance the model training performance. 
\end{itemize}


%We refer readers to for a detailed survey.


%Moreover, some emerging research works not only, data importance aware transmission; transmission power allocation; data retransmission protocol;     



%An intuitive solution is traditional data compression techniques which compress raw data before transmission and decompress raw data after reception. Such data compression can be either lossy compression or lossless compression. 



\textbf{Model Training} - Due to the distributed data and user privacy concerns, distributed training is  suitable for training AI models in a network~\cite{verbraeken2020survey}. FL is one of the most promising distributed training paradigms, which can be applied in various fields such as smart healthcare and financial services~\cite{yang2019federated, lim2020federated, bonawitz2019towards}. The FL operates as follows. Each end user iteratively trains a local model with its own data, and the local model is uploaded to an edge server. Then, the edge server aggregates the local models to obtain a global model. The  model training lasts multiple rounds until the global model achieves satisfactory accuracy.

Since the model is trained locally, FL is communication-efficient and can preserve data privacy of end users~\cite{hard2018federated, li2020federated}. However, with the increase of  data sizes in state-of-the-art AI models,\footnote{The data sizes of ResNet32~\cite{he2016deep}, Inception-v3~\cite{szegedy2016rethinking}, AlexNet~\cite{krizhevsky2012imagenet} and VGG16~\cite{simonyan2014very} models are 50\;MB, 108\;MB, 240\;MB,  and 552\;MB, respectively~\cite{chen2019round}.} uploading local AI models still places a growing strain on spectrum-constrained wireless networks. In addition, end users with powerful computing servers can conduct local model training with a low delay. As such, the model uploading delay due to limited radio resources can be the dominant component in the entire FL delay.  Hence, it is necessary to maximize FL performance in resource-constrained wireless networks.

Recent research works optimize FL performance from the following perspectives: 
\begin{itemize}
    \item \emph{FL Framework Design} - A line of works focus on designing innovative FL frameworks to reduce communication overhead. A novel two-tier hierarchical FL framework is proposed in~\cite{liu2020client}, which coordinates  end users, edge servers, and the cloud server to perform FL. Each edge server aggregates local models from end users in its coverage in every FL round, and the cloud server aggregates the models from edge servers in its coverage once in a few FL rounds. {The proposed two-tier framework can accommodate a large number of end users for model training due to its broad coverage and, at the same time, reduce the backhaul data traffic between the cloud server and edge servers due to a low model aggregation frequency.} Such framework is applied to industrial IoT networks with geographically distributed  data in~\cite{zhang2021dynamic};
   
    \item \emph{Model Aggregation} - Another line of works study radio spectrum-efficient model aggregation. Over-the-air computation based approaches are investigated in~\cite{yang2020federated, amiri2020federated, zhang2021federated}. The basic idea is to exploit the superposition property of wireless multiple-access channels to perform model aggregation, which can reduce radio resource consumption;
    
    \item \emph{Resource Management} - The FL performance can be optimized via efficient resource management. As FL performance depends on multiple factors, such as end user selection, the number of local model updates, and local model importance levels, different resource management schemes are developed as follows: (1) User selection - How to select participating end users in the FL process impacts model convergence and training delay and hence is crucial to FL performance. A few end user selection algorithms are proposed based on principles such as training data distribution~\cite{wang2020optimizing} and local training latency~\cite{nishio2019client}; (2) FL parameters  -  To alleviate communication overhead, end users conduct a few local model updates before model uploading. Given a resource budget, the optimal number of local model updates is studied in~\cite{wang2019adaptive}, which provides a theoretical guideline for selecting the number of local model update; (3) Local model importance level, which is a concept extended from the idea of data importance\footnote{The model importance can be measured by layer-wise gradient norm. Local models with larger gradient norm contribute more to global model convergence in FL~\cite{wang2019adaptive}.} -  An importance-aware model uploading strategy is proposed in~\cite{ren2020scheduling}, in which end users with high   model importance levels and good channel conditions are scheduled with high priority, to speed up the convergence of FL. 
\end{itemize}
 

      
%To solve the issue,  federated learning designs have attracted great attentions from industry and academia. (1) over the air computation, xxx; (2)  coded computation, xxx; (3) resource management, optimize federated learning. (4) architecture design, device-edge-cloud orchestration 


%Unlike FL only utilizes the device's computing resource for model training, split learning is a collaborative model training approach, in which both computing resources from both device and server are utilized. Leveraging the layered structure of DNNs, the entire DNN model is split into a device-side model and a server-side model at a cut layer. Device trains the device-side model, and then the server trains the server-side model. Smashed data and its gradient (small data volume) are transferred between the device and server. Split learning has multiple benefits. Firstly, communication traffic is reduced, since only device-side (partial) model is uploaded for model 

%how it works; its benefits; round robin for multiple user training. 

%model Cascaded 

%PipeDream is prop

%\emph{Model inference} - For many AI services in the network, AI models are usually deployed on end devices and edge servers to achieve low service latency, such as autonomous driving and VR gaming. Conducting model inference is computation-intensive, while either end devices or edge is resource-constrained in both computing capability and battery power. Hence, in addition to inference accuracy, facilitating model inference in the network needs to take service latency and system energy consumption requirements into account, which calls for innovative model inference schemes in different contexts.

%Extensive research efforts have been devoted to develop model inference schemes in different contexts. For low-latency AI services, , AI models can be deployed on the device. Since AI models are computation-intensive, conducting model inference on the device usually requires powerful on-device computing facility and sufficient battery capacity, which makes it difficult to be deployed at low-end devices.




\textbf{Model Inference} - For many AI services in the network, AI models are usually deployed at end users and edge servers to achieve low service latency. The model inference is computation-intensive, while end users and edge servers usually have limited computing capabilities and battery power. Executing model inference tasks usually results in long service latency and  high energy consumption. Hence, performing model inference should satisfy service latency under node energy constraints, thereby calling for innovative model inference schemes.

Existing studies on model inference can be categorized as follows: 
\begin{itemize}
    \item \emph{Data Resolution} - Raw data are offloaded to edge or cloud servers for model inference. The input data resolution influences the inference accuracy. For instance, the accuracy of object detection  is related to the input image resolution~\cite{liu2018edge}, which in turn affects the offloaded data volume since the data size of high-resolution images is usually large. Taking into account the trade-off between the inference accuracy and the amount of offloaded data, the input image resolution should be optimized to satisfy the target AI service requirements. The optimal video frame rate and input image resolution are investigated in~\cite{liu2018edge} to balance service latency and detection accuracy for virtual reality users;
    
    \item \emph{Model Selection} -  An appropriate AI model is selected to satisfy specific AI service requirements. In addition to the data resolution, the inference accuracy depends on the type of AI models. A DNN model with more hidden layers can usually  achieve a higher inference accuracy than a shallow DNN model. Considering multiple available DNN models deployed at the network edge, the optimal DNN model selection  for real-time video analytics is investigated in~\cite{wang2020joint};
    
    \item \emph{Model Partition} - With advanced model partition techniques, an AI model can be partitioned into multiple sub-models and then embedded into different network nodes to conduct model inference. For instance, leveraging the layered structure of DNNs, the entire DNN model can be partitioned into an end user-side model and a server-side model at a proper DNN layer (i.e., the cut layer). As such, the end users and the edge servers can conduct model inference in a collaborative manner. DNN models can be partitioned for achieving different goals. For instance, the optimal model partition for minimizing inference latency is studied in~\cite{zhang2021autodidactic}, in which an online learning algorithm can adaptively determine the optimal cut layer. To reduce communication overhead among network nodes, complicated DNNs models can be partitioned into sub-models for end users, edge servers, and the cloud as in~\cite{teerapittayanon2017distributed};
    
     \item \emph{Model Compression} - Light-weight models are used to facilitate prompt model inference at end users. Computation-efficient compressed models can be obtained via various model compression techniques, such as weight pruning~\cite{han2015deep}, knowledge distilling~\cite{chen2017learning} and fast exiting~\cite{teerapittayanon2016branchynet}. For instance, weight pruning techniques remove less important model weights to reduce the  computational complexity of model inference, while achieving inference accuracy close to that of the uncompressed models. To enhance service performance, a collaborative model inference scheme that deploys light-weight models at IoT devices and uncompressed models at the network edge is proposed in industrial IoT networks~\cite{wu2020accuracy}. The IoT devices dynamically make AI task offloading decisions according to time-varying channel conditions to minimize the service delay while guaranteeing the accuracy requirements of DNN-based fault diagnosis services.
\end{itemize}



%suffer from  computing resource   
%The model inference can be conducted on the device. 

%model inference, model partition, model pruning, 

%model-variant selection based on channel condition, infocom and han tao; 

%1. on device design, 1. architecture, 2. resource management 


\begin{figure*}[h]
	\centering
	\renewcommand{\figurename}{Fig.}
	\includegraphics[width=0.9\textwidth]{Fig/fig5.pdf}
	%	\vspace{0cm}
	\caption{Conceptual AI slice consisting of a training subslice and an inference subslice.}
	\label{fig:slicing_for_AI}
\end{figure*}



\subsubsection{Research Challenges}\label{subsubsec: challenges}
% The following discussion on networking techniques for AI uncovers fundamental research challenges that confront networking and inhibit wide deployment of AI services. 
 
Despite the aforementioned research efforts, facilitating AI services in a network faces various challenges, some of which are discussed in the following.
%\subsubsection{AI Service}
% After training, the model is deployed to conduct online inference. %Both model training and model inference are important for implementing AI services.  
%Both model training and model inference consume a large amount of computing, storage, and communication resources. 


%Decentralized training is a promising training manner in wireless networks due to the following reasons: (1) low communication cost - Sending all the data to a centralized node incurs prohibitive communication cost, e.g., a single autonomous driving vehicle can generate more than one Gigabit data per second; and (2) preserving data privacy - Offloading data to a centralized node renders user privacy concerns since the data capture user behaviours. To implement decentralized training, the following iterative procedure is conducted, including: i) a centralized node distributes a global model to all attending users; ii) each user trains the model based on its data and then sends the trained local model to the centralized node via communication links; and iii)  the centralized node aggregates all the local models to generate a new global model~\cite{mcmahan2017communication}, as shown in Fig.~\ref{fig:slicing_for_AI}.




\emph{Complex Implementation Option Selection} - An AI service can be implemented by various options with different model structures, training procedures, and inference processes. For instance, a service of object detection can be implemented via different neural networks, such as AlexNet~\cite{krizhevsky2012imagenet} and SqueezeNet~\cite{iandola2016squeezenet}. Even if the model structure is the same, a model can be trained in different ways, such as centralized training, decentralized training (e.g., FL~\cite{yang2019federated}), and semi-centralized training (e.g., split training~\cite{thapa2020advancements}). In addition, model inference can be conducted in various manners, such as end user-only inference, edge-only inference, and collaborative inference. Different implementation options consume different amounts of computing, storage and communication resources. Hence, it is necessary to select an implementation solution for AI services that suits the service characteristics and network dynamics.    	 

%\emph{Inefficient model training} - AI services have a unique focus on model training. Carrying out model training in networks has different implementation options which face different issues. Taking decentralized training for example, its performance in networks is significantly throttled by several issues: (1) {Straggler effect} - Due to user heterogeneity, users with limited communication bandwidth or insufficient computing powers, namely stragglers, take more time to complete local model training than others~\cite{lim2020federated, yang2019federated}. Other users have to wait for stragglers, which significantly slows down the model training process; (2) Communication cost - Decentralized training systems need to exchange model parameters for many (up to hundreds) training rounds until convergence. Extensive model parameter uploading from end devices to edge servers places a heavy burden on the network, which renders communication as a bottleneck. Due to constrained communication resources in networks and ever-increasing size of advanced AI models, parameter uploading may take a long time. Hence, enabling efficient model training is desired;


\emph{Multi-Dimensional QoS Requirements} - The QoS requirements of AI services are multi-dimensional.  AI model accuracy is usually a key performance metric. In addition, AI services should be offered to end users with low latency in many use cases. For instance, the service latency of object detection in autonomous driving should be less than 100\;\emph{ms} for safety considerations~\cite{lin2018architectural}, whereas autonomous vehicles require an ultra-high accuracy in 3D object detection~\cite{chen2017multi}.  Moreover, these performance metrics are correlated. High-accuracy object detection usually requires high-resolution images as input and advanced AI models to process the input images, which can result in long service latency. How to satisfy multi-dimensional QoS requirements of AI services requires further investigation.

%The impact of mobility



%\item Diversified implementation algorithm
%	\item resource limited 
%\end{itemize}
%In summary, AI services 



%It is expected that many AI services will emerge in the coming future. To support these AI services with different QoS requirements, new slices are established for emerging AI services, named \emph{AI slices}. \emph{Slicing for AI} is to design network slices to support AI services. 

%Intelligence-as-a-service (IaaS) is important, especially in edge networks, such as objection systems



%Challenges: straggler effect




%Moreover, training performance depends on the resource availability and data availabilities at all network nodes. 


%----------------------------------------------------------------------------------------------------
%\subsubsection{AI Instance}\label{subsec:AI_instance}
%\begin{figure*}[h]
%	\centering
%	\renewcommand{\figurename}{Fig.}
%	\includegraphics[width=0.7\textwidth]{Fig/fig6.pdf}
%	%	\vspace{0cm}
%	\caption{The AI instance concept for flexible AI service management.}
%	\label{fig:AI_instance}
%\end{figure*}

%To address the challenge that AI service 

%In the following, we propose an AI instance framework to facilitate flexible AI service management. An AI instance represents an implementation option of the AI service. The framework is designed to provide AI services via selecting appropriate implementation options, i.e., selecting appropriate AI instances. As shown in Fig.~\ref{fig:AI_instance}, the detailed operation of the AI instance framework consists of two steps:
%\begin{itemize}
%	\item {AI Instance Construction}: The network operator creates multiple candidate AI instances for each AI service based on available virtualized network resources. Specifically, an AI instance is composed of multiple attributes, including: (1) algorithm type, which specifies the implementation algorithm and its neural network architecture (e.g., the number of neural network layers, and activation functions in each neural network layer); (2) training manner, which specifies the training manner of the specified implementation algorithm; and (3) required network resources, which specifies not only the amount of network resources (including communication, storage and computation resources) for both training and inference, but also the physical locations of the network resources; %Even if the amount of consumed network resources is the same, different implementation algorithms may consume network resources from different physical locations. %Due to different attributes, the same AI service can have multiple implementation manners, i.e., multiple AI instances for its implementation. 
%	\item {AI Instance Selection}: This step is to associate the AI service provider with its appropriate AI instance. For this purpose, the AI service provider observes the status and collects requirements from its current subscribed users, and then selects an AI instance among candidate AI instances provided by the network operator. The collected user status may include the computing capabilities of users, which affects the model inference stage. High-end end users with considerable computing capability can handle high local computation workloads, which prefers device-only inference, and while low-end end users prefer collaborative inference. The collected user requirements can include the desired privacy level. The privacy level has an impact on the selection of training mode. Decentralized training, semi-centralized training and centralized training are preferred for high, middle and low privacy levels, respectively.
%\end{itemize}


%The proposed AI instance concept aims to facilitate {flexible AI service management}. The network operator can dynamically manage AI services via creating, modifying and deleting candidate AI instances on demand, to reduce complexity in AI service management. 

%; and (2) \emph{service data privacy preserving} - In the framework, each AI service provider selects its own AI instance without sharing its subscribed users' information with the network operator, thereby preserving service data privacy.


%{user-centric AI service} - The AI instance selection is conducted based on the current users' status and requirements, such as privacy level and device computation capability, and hence network resources including device's resources (e.g., on-device computing capability) can be efficiently utilized; and

%With AI instances, we propose an \emph{AI instance based service management framework}. The basic idea is that each 

%The detailed procedure is given as follows. Firstly, 
% Secondly, Thirdly, the AI service provider selects the optimal AI instance based on the collected information.


%In summary, addressing the preceding challenges is essential to facilitate AI services in the network. 

%----------------------------------------------------------------------------------------------------


\subsubsection{AI Slice}\label{subsec:AI_slice}\label{subsubsec: AI_slice}
To better support AI services, we extend the network slice concept and propose an idea of \emph{AI slice} with two subslices. The basic idea is to construct a \emph{training subslice} for model training and an \emph{inference subslice} for model inference. The two subslices are logically isolated and use their own network resources. The rationale behind training and inference separation is that the two stages can have different goals.% For instance, the model inference stage should achieve low inference latency, while the model training stage should achieve high model accuracy. 



%The training stage  (e.g., decentralized training) may require coordination among network nodes (e.g., end users), {while the inference stage can be individually performed at each network node (may be incorrect)}. %As such, two stages are relatively independent, which should be implemented via two subslices.

{An illustration of an AI slice is given in Fig.~\ref{fig:slicing_for_AI}. In the AI slice, the training and inference subslices share the same resource pool and are coordinated to jointly support the AI service. First, the multi-dimensional QoS requirement of the AI slice is decoupled into two separate QoS requirements for the two subslices. For an object detection service in autonomous driving, both high detection accuracy (e.g., 99\%) and low service latency (e.g., 100\;\emph{ms}) are required. The training subslice should satisfy the detection accuracy requirement, while the inference subslice should satisfy the service latency requirement. Second, to satisfy the individual QoS requirements of the two subslices, the resources reserved for the AI slice are judiciously allocated between the two subslices, based on the performance of the two subslices and their QoS requirements. Then, given the allocated resources, the two subslices are configured to satisfy their individual QoS requirements, as described in the following: }
\begin{itemize}
    \item In the training subslice, based on the training data distribution in the network, a subslice controller determines training configurations (e.g., data collection schemes and model training methods) and schedules resources to network nodes to train a model given the target accuracy. In addition, since the training data vary over time in a dynamic network, the AI model may need to be retrained from time to time. Note that allocating dedicated resources for the training subslice can effectively mitigate the straggler effect that plagues distributed learning in large-scale networks, thereby speeding up the model training process;
    
    \item In the inference subslice, the subslice controller analyzes the service  demand pattern at each BS and  determines inference configurations (e.g., model inference and input data compression schemes) to satisfy the inference latency requirement. For instance, uncompressed models can be deployed at resource-abundant BSs, and partitioned and pruned models can be deployed at resource-limited BSs. This can achieve close inference service latency performance across different BSs.
\end{itemize}
{Overall, the two logically-isolated subslices focus on satisfying different QoS requirements and jointly support the AI service.}

%  Specifically, the training subslice aims to satisfy the model accuracy requirement, and the inference subslice aims to satisfy the service latency requirement. %The coordination between them can satisfy multi-dimensional QoS requirements of AI services.


To elaborate the idea of AI slices, we present the following example on real-time video analytics in vehicular networks~\cite{wang2020joint}. Smart cameras are deployed in  intersections to provide a video surveillance service such as vehicle plate recognition. In such service, a CNN model is trained using the video streams collected by smart cameras, and then the well-trained model is used to conduct video analytics tasks. Using the proposed AI slice framework, CNN model training is conducted in a training subslice, while real-time video analytics is conducted in an inference subslice. Specifically, in the training subslice, the CNN model can be trained via a FL framework for protecting data privacy. The corresponding computing resources at smart cameras and spectrum resources in the network are allocated to satisfy model training requirements, such as training accuracy. In the inference subslice,  different user-edge orchestration schemes (e.g., DNN model partition), input data compression schemes (e.g., frame rate reduction), and network resource management policies can be configured to satisfy the inference delay requirement in video analytics services based on time-varying service demands and network conditions due to vehicle mobility. With the AI slice for video analytics, both training accuracy and inference latency requirements can be satisfied in a dynamic network environment. 


\subsection{{Summary}}
{In this section, we have reviewed some common AI techniques, explored the role of AI in 6G networks, and proposed a four-layer AI architecture for pervasive intelligence in 6G. Two perspectives of AI in wireless networks, i.e., AI for networking and networking for AI,  have been discussed, which correspond to using AI as a powerful tool for network management and optimizing networks to support AI applications, respectively. }

{Recent advancements in ML algorithms have accelerated the deployment of AI in wireless networks. In 5G, AI techniques are used to address particular networking problems, whereas, in 6G, AI will penetrate every corner of wireless networks from network management to network services. Therefore,  an architecture for AI is needed for identifying the role of AI and characterizing the functionalities of AI across a network.}

Appropriate AI techniques should be selected to tackle networking problems with different characteristics and on different decision time scales when it comes to AI for networking. Furthermore, the collaboration among intelligent modules is important to implement AI-driven networks efficiently and flexibly. The idea of connected AI is to enable cooperative decision making among intelligent modules for network control. In terms of networking for AI, a distributed architecture of AI algorithms connects AI models and network resources located at network edge. The study of networking for AI is still in its infancy but essential to supporting an expanding group of AI services. Network slicing will remain to be an enabler for delivering AI services, but slicing policies should be customized according to the features of AI algorithms and the training and inference stages of AI.

%Building on the vision of holistic network virtualization and pervasive network intelligence, an overall network architecture for 6G networks is proposed in the next section.

% \space


==> Final version/sec_Propose_Network_Architecture.tex <==
 \begin{figure*}[t]
	\centering
	\renewcommand{\figurename}{Fig.}
	\includegraphics[width=0.95\textwidth]{Fig/fig7.pdf}
	%	\vspace{0cm}
	\caption{The proposed network architecture for 6G networks.}
	\label{fig:proposed_architecture}
\end{figure*}


In this section, we propose a conceptual network architecture for 6G, which integrates holistic network virtualization (including digital twins and network slicing) and pervasive network intelligence (including connected AI and AI slices). Then, we illustrate three types of interplay enabled by the proposed architecture, i.e., the interplay between digital twin paradigm and network slicing, model-driven methods and data-driven methods, and virtualization and AI, respectively.  


\subsection{Related Studies on Architecture for 6G} \label{ss:related6Garc}
Several works have proposed architectures with various focuses for 6G networks, e.g., space-air-ground integrated networks for global coverage~\cite{M_NZhang}, cell-free massive multiple-input multiple-output (MIMO) architecture for inter-cell interference mitigation~\cite{ngo2015cell}, and multi-tier computing architecture for ubiquitous computing service provisioning~\cite{yang2019multi}. Pursuing the goal of advanced network management, most of the proposed architectures highlight AI techniques to optimize network architecture, control, and management~\cite{M_KLetaief2019, itu2019architectural}. For example, AI-based data analytics functions, which mine historical data for network operation troubleshooting, network resource optimization, and network traffic prediction, are incorporated in the network architecture in ~\cite{M_KLetaief2019}. The ITU specifies a high-level AI-based architectural framework for future networks, in which several novel components such as ML management and orchestration functionalities are incorporated for flexible AI-based function placement~\cite{itu2019architectural}. In addition to AI techniques, some recent conceptual network architectures start to embrace digital twin techniques~\cite{M_Q_Yu_2019, khan2021digital}. For example, a digital twin-based network architecture constructs a digital twin for each end user to serve as its communication assistant and data asset manager~\cite{M_Q_Yu_2019}. Another digital twin-enabled network architecture adopts three categories of digital twins, i.e., edge-based, cloud-based, and hybrid  digital twins, for supporting different types of services~\cite{khan2021digital}.

Different from the existing network architectures, our proposed network architecture features novel holistic network virtualization, which incorporates network slicing and digital twin paradigms, and pervasive network intelligence, which integrates AI for networking and networking for AI. Moreover, featuring the designs in Sections~\ref{sec:HNV}~and~\ref{sec:PI}, the proposed architecture enables various interplay among its key elements to empower 6G. In the following subsections, we present the details of the proposed architecture.


\subsection{Architecture Overview}\label{ss:ArcOv}




% In addition, detailed network components and potential implementation of the proposed conceptual architecture have been discussed.  


The overall network architecture is illustrated in Fig.~\ref{fig:proposed_architecture}, which consists of the physical space and the cyber space. The physical space includes end users and network infrastructure at the edge and the core networks. Data describing end users are collected from the physical network to create level-one digital twins as introduced in detail in Subsection~\ref{ss:HNV}, and network slices are created for various services. The slices are further abstracted into level-two digital twins, which are supplemented with service-specific information aggregated from level-one digital twins. The six-layer virtualization architecture in Fig.~\ref{fig:digital_twin} applies to the network slices and the digital twins, both of which reside in the cyber space in Fig.~\ref{fig:proposed_architecture}.

AI pervades the entire architecture, which supports both AI for networking and networking for AI. First, AI is used to manage network slices and digital twins, as shown in the logic network control section in Fig.~\ref{fig:proposed_architecture}. For network management, a connected AI solution discussed in Subsection~\ref{ss:AIforNet} is applied to enable intelligent modules, which in turn manage network slices and digital twins. The connected AI solution corresponds to AL 3 and 4 in Fig.~\ref{fig:1}. Second, the  architecture supports dedicated AI slices with training and inference separation for AI service provisioning, as mentioned in Subsection~\ref{ss:NetforAI}. AI slices provide services corresponding to AL 1 and 2 in Fig.~\ref{fig:1}, while the management of AI slices is conducted by intelligent modules.  

With the overall network architecture in Fig.~\ref{fig:proposed_architecture}, we integrate holistic network virtualization and pervasive network intelligence for 6G. Virtualization is supported from the aspects of both the network and the end users, while intelligence is reflected through both AI for networking and networking for AI. Taking advantage of digital twin paradigm and network slicing as well as those of virtualization and AI, the proposed architecture aims at exceeding flexibility, scalability, adaptivity, and intelligence. 

\subsection{Components and Subsystems}\label{ss:comp}

In the physical space, the proposed architecture includes both RANs and core networks. Specifically, the following components are involved:
\begin{itemize}
    \item Assorted APs: This component includes MBSs, SBSs, mobile APs (such as UAVs), satellites, and other non-cellular APs; 
    \item Network controllers: This component includes local controllers located at APs or servers on  network edge and the centralized controller located at servers in core networks or in the cloud. Each controller can consist of computing servers and affiliated network storage servers;
    \item General computing servers: This component includes computing servers for implementing network functions, such as routing and firewall, and hosting the VNFs;  
    \item Application servers: This component includes computing and network storage servers for supporting general edge computing and AI services. These servers are not used for  network management or implementing network functions;   
    \item Other network devices: This component includes specialized network hardware that are not general computing servers, such as baseband processing units and network switches;
    \item End users: This component includes human mobile users, sensors, vehicles, and various IoT devices, such as meters, actuators, and robots. 
\end{itemize}
In the cyber space, the proposed architecture includes three subsystems, i.e., network slices, digital twins, and connected AI, as follows:
\begin{itemize}
    \item Network slices: This subsystem includes all virtual networks created in network slicing, including AI slices. A network slice can involve a RAN, a core network, or both. General slices are inherited from existing networks, while AI slices are described in detail in Subsection~\ref{ss:NetforAI};   
    \item Digital twins: This subsystem includes level-one and level-two digital twins. The digital twin subsystem is described in detail in Subsection~\ref{ss:HNV};
    \item Connected AI: This subsystem includes intelligent modules deployed across a network at both the local controllers and the centralized controller. The connected AI subsystem is described in detail in Subsection~\ref{ss:AIforNet}.  
\end{itemize}
Interconnections between different components and subsystems of the proposed architecture are elaborated in Subsections~\ref{ss:IntDTNS}~to~\ref{ss:IntVTAI}, which highlight the interplay between digital twin paradigm and network slicing, between model-driven and data-driven methods, and between virtualization and AI, in the proposed architecture. Some open issues and challenges regarding the architecture are presented in Section~\ref{sec:Open}. 

Note that the proposed conceptual architecture can apply to various types of physical networks, such as vehicular networks and integrated terrestrial-satellite networks, although Fig.~\ref{fig:proposed_architecture} cannot illustrate every possible network scenario. In different physical networks, the implementation of holistic network virtualization and pervasive network intelligence can be different and require certain customization. For example, the deployment of intelligent modules and the data flow among the modules in a satellite network segment can be different from those in a terrestrial network segment. Furthermore, the migration of digital twins can be more important in a vehicular network than in a static IoT network. Related discussions can be found in Section~\ref{sec:Open}, where we present challenges and open issues. Nevertheless, the basic ideas in the proposed conceptual architecture, including the two-level digital twins, intelligent modules, and AI slices, are applicable in various physical networks.

\subsection{Implementation\label{ss:Implement}}
In this subsection, we provide a case study on a vehicular network to demonstrate the potential implementation of the proposed network architecture. Roadside BSs co-located with edge computing and caching servers facilitate autonomous driving services for vehicles on the road. To implement the proposed network architecture, the following steps are conducted.

\begin{itemize}
    \item \emph{Network Slice Establishment}: Multiple network slices are established  for autonomous driving services with different QoS requirements, achieving network virtualization. Conventional network slices are established for non-AI based services, e.g., high-definition map downloading, while AI slices consisting of training and inference subslices are established for AI based services, such as deep learning based cooperative sensing. The network slices are stored and managed by a centralized controller.
    
    \item \emph{Digital Twin Construction}: By collecting extensive data from  physical entities, digital twins are constructed for vehicle users, roadside BSs, and the established network slices, achieving the virtualization of end users and slices. Digital twins of vehicle users and roadside BSs are located at edge servers, while digital twins of network slices are located at a cloud server. Due to high vehicle mobility, digital twins of vehicle users should be migrated across edge servers to ensure service continuity. In addition to collected data, digital twins can include generated user and service specific data, such as predicted vehicle trajectory and spatial-temporal service demands, via mining historical data. The generated vehicle data will be used for network management and service provision.
    
    \item \emph{AI Module Deployment}: AI modules with different functionalities can be deployed at both the centralized and local network controllers, achieving intelligent network management. The AI modules at the centralized network controller are in charge of network planning. For guaranteeing QoS requirements of different slices, these AI modules can make resource reservation decisions based on the predicted service demands from the digital twins of roadside BSs and collected slice performance data from the digital twins of network slices. The AI modules at local network controllers are in charge of network operations. For enhancing the perceived performance of the vehicle users, the AI modules schedule on-demand network resources based on the collected data (e.g.,  vehicle users' channel conditions) and the generated data (e.g., predicted vehicle trajectory) from the digital twins of vehicle users. 
    
    % at each BS predicts slice traffic demand via advanced AI-based traffic prediction algorithms~\cite{gutterman2019ran}. Based on the collected information, the cloud-hosted AI module adaptively adjusts provisioned network resources for slices. 
    
    % (2) Network operation - Network operation decisions are made by the network-hosted AI module at the local controller which collects the following network information, including real-time network information collected by digital twins (e.g., end user channel conditions) and the predicted user information generated from digital twins (e.g., predicted user trajectory).
\end{itemize}


% In the considered case, network slices are established on the vehicular network to support autonomous driving services, and digital twins are constructed for network slices and physical entities (including vehicle users and RSUs) in the network, which enables holistic network virtualization. The operation workflow is as follows.

% \begin{itemize}
    % \item \textcolor{magenta}{\emph{Data collection for digital twins}: This step is to collect real-time data from physical network and network slices for different types of constructed digital twins. (1) End user digital twins located at edge servers collect connectivity-related information (e.g., channel state information and location/speed) and service-related information (e.g., user service demand request and service satisfaction). Such data collection is coordinated by the local network controller that end user digital twins associated with, which schedules communication resources for data collection based on the configured data attributes and collection frequencies. (2) Network infrastructure digital twins located at edge servers collect service traffic load information and available resource information. Such data collection is also conducted by the local network controller. (3) Network slice digital twins located at the cloud server collect the monitored slice performance information, which is coordinated by the centralized network controller.} 
    
    % \item \textcolor{magenta}{\emph{Data generation from digital twins}: This step is to generate specific data and information from constructed digital twins for facilitating advanced network management. (1) User-specific data can be obtained from end user digital twins by mining extensive collected historical data, such as predicted vehicle user trajectory and estimated user service request pattern. (2) Service-specific data can be obtained from network infrastructure digital twins. For example, the spatial-temporal service demand information can be predicted based on service traffic load information.} 
    
    % \item \textcolor{magenta}{\emph{Network management decision making}: This step is to make network management decisions leveraging the collected and generated information from digital twins.}
% \end{itemize}








\subsection{Interplay between Digital Twin Paradigm and Network Slicing}\label{ss:IntDTNS}

As the two components of holistic network virtualization, digital twin paradigm and network slicing are connected in the following two aspects.

First, the digital twin paradigm for end user virtualization focuses on data management, while network slicing focuses on network management. Data may be viewed as a new type of resources in future networks, in addition to communication, computing, caching, and sensing resources. Meanwhile, as a resource, data has its unique features. First, data can be considered as an application-layer resource rather than a physical-layer resource. Second, different from computing or communication resources, the amount of data resources available to a network is not fixed but progressive. Last, the collection and processing of data, which is necessary for utilizing any data resource, consume other network resources. On one hand, effectual utilization of the data resource will benefit network management, and hence digital twin paradigm can enhance network slicing. On the other hand, network management should take into account the need and cost of allocating other network resources for utilizing the data resource. Hence, network slicing can facilitate digital twins.      

Second, digital twins will enable user-centric networking in future networks, while network slicing enables service-centric networking. Creating an isolated slice for each service and provisioning the service through managing the slice yield a service-centric focus in network management. Meanwhile, creating a digital copy of each end user and administrating data that characterize the end user provide a user-centric perspective of network management. Having a set of information, selected by the centralized controller through digital twin model control, to describe various characteristics of the end users, such as their location, service request profile, resource utilization, and channel information, creates the possibility of user-specific scheduling within each slice in the network operation stage. For instance, access control and resource allocation decisions for an end user may depend on the data profile from its digital twin, while different data profiles may lead to different scheduling policies.  Accordingly, future networks may feature service-centric network planning and user-centric network operations, which can improve the granularity of network management for handling highly diversified end users and dynamic network environments.



% \subsection{Integration}
 
%  interplay
%  data: DT --> AI, AI (management) --> DT, AI (application) --> DT (behavior prediction data)
%  resource sharing: computing resource (network management), joint orchestration; updating (bandwidth); caching (storage);  control resource or data resource
%  model:  
 
 
%  interface
%  2 levels DT --> 4 Level AI, data flow 
 
% ------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------

% \subsection{Implementation}
% In this subsection, we present a detailed case of network slicing to have a better understanding of implementing advanced network management via AI and virtualization. 

% As mentioned in Section~II, network slicing consists of two stages: network planning and network operation~\cite{J_XShen_2020}. Specifically, the {network planning} stage operates in a large time scale (from minutes to hours) to provision network resources for multiple slices to guarantee their service level agreements. The {network operation} stage operates in a small time scale (e.g., 100\;\emph{ms}) to orchestrate the provisioned network resources of a slice among its subscribed end users. In both two stages, AI modules and digital twins are operated in synergy. The detailed procedure is given as follows.
% \begin{itemize}
% 	\item {Network planning:} The cloud-hosted AI module at the global controller is in charge of network planning. The AI module collects information from digital twins and AI modules resided at other levels. Specifically, the level~two digital twins abstracted from network slices provides service-specific data (e.g., historical slice performance data), and the edge-hosted AI module at each BS predicts slice traffic demand via advanced AI-based traffic prediction algorithms~\cite{gutterman2019ran}. Based on the collected information, the cloud-hosted AI module adaptively adjusts provisioned network resources for slices. 
	
% 	\item {Network operation:} Network operation decisions are made by the network-hosted AI module at the local controller which collects the following network information, including real-time network information (e.g., users' channel conditions), user-specific data from the level~one digital twins (e.g., user mobility), and the predicted user information from device-hosted AI modules (e.g., predicted user trajectory).  
% \end{itemize}


\subsection{Interplay between Model-Driven and Data-Driven Methods}\label{ss:codriven} \label{subsec:Model-data Co-driven}

The second interplay enabled by the proposed architecture is the interplay between model-driven and data-driven methods in network operation and service provision. This interplay applies to the intelligent modules for network management shown in Fig.~\ref{fig:proposed_architecture}.

Network management mostly relied on model-driven or heuristic methods before 5G. Prior to the prevalence of AI, mathematical tools such as optimization methods and game theory have been widely used for network management. Optimization methods formulate the objective and constraints in a closed form, and the corresponding network management problems are solved using optimization algorithms~\cite{Mushu_UAV, Leconte,Halabian}. Game-theoretic approaches analyze the interactions among network entities in either cooperative or non-cooperative scenarios to identify  the optimal strategy of each entity~\cite{Xiong1, Xiong2, Caballero}. Mechanism design, an analytical framework in game theory, has also been used to coordinate network entities with locally-held information to achieve desirable network-wide solutions in network utility maximization problems~\cite{J_Jie_MD_2018}.    


%\textcolor{blue}{When forming a game, the utility functions for network entities participating in the game should be obtained, while obtaining the functions may not be feasible when network environments and relationships among network entities are complex. AI techniques can provide potential solutions to the challenges posed by optimization and game theory in resource management. Advanced machine learning methods can be applied in resource management to efficiently predict network traffic, make network management decisions, and identify the complex relationships among network entities.}

Through characterizing the relations among several key variables, model-driven methods can lead to either closed-form solutions or algorithms for network management problems. Based on mathematical models, model-driven methods are usually explainable and generalize well for different specific problems~\cite{zappone2019wireless}.\footnote{For instance, the water-filling algorithm could be applied to various power allocation problems, and the Rayleigh fading model could characterize channels in various network environments.} However, when networks become complex (i.e., when there are a large number of variables and/or complicated correlation among them) or highly dynamic (e.g., when the network environment changes too rapidly for an optimization algorithm to converge or for a game to achieve an equilibrium), model-driven methods may no longer be accurate or applicable. 

The investigation of data-driven methods for network management has gained momentum since 5G. Through collecting and exploiting real-world data, data-driven methods implicitly characterize the relations among variables to generate and fine-tune policies for network management. Given sufficient data and a stationary network environment, data-driven methods can provide close-to-optimal solutions to problems that are too complicated for model-driven methods. However, when the network environment is non-stationary so that new and unknown situations occur from time to time, the performance of data-driven methods can be questionable~\cite{yang2020deep}. In addition, data-driven methods may not generalize well due to their strong dependence on data collected from a specific network environment.             

In 6G, data-driven and model-driven methods should work in synergy. The proposed architecture enables the interplay between data-driven and model-driven methods for creating advanced \emph{hybrid data-model driven} methods. There are different options of hybrid data-model driven methods, as illustrated in Fig.~\ref{fig:HDMD} and elaborated below. The first three options suit AI for networking, while the last option suits networking for AI.   

\begin{figure}[t]
	\centering
	\subfloat[Backup/switching]{
		\includegraphics[width=0.36\textwidth]{Fig/fig10_1.pdf}\label{fig:HDMD1}}\\
		\vspace{-3mm}
	\subfloat[Task division]{
		\includegraphics[width=0.36\textwidth]{Fig/fig10_2.pdf}\label{fig:HDMD2}}\\
		\vspace{-3mm}
	\subfloat[Refinement]{
		\includegraphics[width=0.36\textwidth]{Fig/fig10_3.pdf}\label{fig:HDMD3}}\\
		\vspace{-5mm}
	\subfloat[Mixing]{
		\includegraphics[width=0.36\textwidth]{Fig/fig10_4.pdf}\label{fig:HDMD4}}
	\caption{Options for hybrid data-model driven methods. The ``Data'' and ``Model'' blocks represent ``data-driven methods'' and ``model-driven methods'', respectively. }
	\label{fig:HDMD}
\end{figure}

\begin{itemize}
    \item \emph{Backup/Switching} - Data-driven and model-driven methods can be the backup for each other. For instance, models can be selected to back up data-driven methods, for the case when unknown situations occur in the network environment and degradation in the performance of data-driven methods appears. Meanwhile, switching between data-driven and model-driven methods, e.g., based on the available resources, can potentially increase the adaptivity of network management. 
    %the availability of data and intelligence everywhere in the proposed network architecture allows AI modules to run in the background to back up model-driven methods, for the case when a mismatch between the expected and the actual performance of any chosen model is observed. 
    \item \emph{Task Division} - Date-driven and model-driven methods can target different steps and solve different subproblems of network management. Specifically, data-driven methods can solve the subproblems with a large number of variables or complicated coupling relations among variables, while model-driven methods can solve relatively isolated subproblems with a few key variables. This would allow data-driven and model-driven methods to play to their respective strengths.   
    \item \emph{Refinement} - Model-driven methods can provide rough solutions based on general mathematical models, and then data-driven methods, taking the rough solutions as input and exploiting real-world data from the network, can refine the solutions for the specific network scenario. Having the initial solution generated from models may reduce either the amount of data or the amount of time needed by data-driven methods.      
    \item \emph{Mixing} - In networking for AI, while deploying a service function chain for an AI service, some of the function modules can use data-driven methods, while other function modules in the same service function chain can use model-driven methods. For example, in an AI-based image processing service, a model-driven module can be used for image resolution adjustment prior to a data-driven module for object detection. The idea is similar to task division, except that the scenario here is networking for AI instead of AI for networking  \cite{li2021slicing}.
\end{itemize}






\subsection{Interplay between Virtualization and AI}\label{ss:IntVTAI}
The third interplay enabled by the proposed architecture, i.e., the interplay between virtualization and AI, is illustrated in Fig.~\ref{fig:digital_twin_AI}. 

First and foremost, virtualization and AI are coupled through data. With the introduction of digital twins, a vast amount of organized data regarding end users, i.e., level-one digital twins, and network services, i.e., level-two digital twins, become available. The data included in the digital twins can be provided to the intelligent modules, the training or inference subslice of an AI slice, or both. For instance, edge-hosted AI, possibly collaborating with end user-hosted AI, can perform user-specific data processing and prediction based on the data from digital twins. The results, such as prediction results, resource scheduling schemes, or slicing policies, can be fed back to the digital twins to record certain predicted status, e.g., location and mobility, of the end users. Correspondingly, data in the digital twins of end users, network infrastructure, and slices can be either the input or the output of AI modules, leading to a bidirectional interaction between virtualization and AI.\footnote{Interested readers are referred to~\cite{S_DC.Nguyen_ST_2021} for the relation between AI and data life cycle, although the discussions therein do not involve virtualization.}

The second connection between virtualization and AI is through control. Based on the data from digital twins, AI  functions hosted at the edge and core networks can make the network management and service provisioning decisions. The decisions may include network slice control, which are fed back to the physical network and network slices for execution and, at the same time, to the level-two digital twins for data update. In addition, the decisions may include digital twin model control for level-one and level-two digital twins. Digital twin model control may include the determination of the type and the amount of data to be included in digital twins, the frequency and the method of data collection, the format and the precision of stored data, and so on. The digital twin models affect the availability and quality of data available for network control, especially AI-driven network control, and thereby impact the network performance. Therefore, from the perspective of network control, the interaction between virtualization and AI is also bi-directional.\footnote{The interaction between digital twin and AI for intelligent network control is discussed in~\cite{O_Zhou_IETF21}. Note that the definition of digital twins therein is different from ours.}        

\begin{figure}[t]
	\centering
	\renewcommand{\figurename}{Fig.}
	\includegraphics[width=88mm]{Fig/fig8.pdf}
	%	\vspace{0cm}
	\caption{Interplay between virtualization and AI.}
	\label{fig:digital_twin_AI}
\end{figure}


The third and implicit connection between virtualization and AI is through resources. Holistic network virtualization requires extensive resources, including computing resource for virtual network functions, caching resource for storing digital twins, and communication resource for the synchronization between end users and their digital twins. Similarly, pervasive network intelligence also requires extensive computing resource and possibly other resources, e.g., communication resource for distributed training as mentioned in Section~\ref{sec:PI}. Therefore, the network resources need to be shared and coordinated between virtualization and AI functions. However, this does not mean that virtualization and AI functions simply compete for resources. Instead, they can help each other improve resource utilization efficiency. %It might be possible to implement certain virtual network functions, e.g., policy control or protocol selection, via the inference part of AI. 
%The corresponding training phase can be optimized in a centralized fashion to reduce computing resource consumption. 
Digital twin paradigm may reduce the resource consumption of AI functions by providing high-importance data only. This can be achieved by the aforementioned digital twin model control. Meanwhile, creating a digital twin for every end user may be too resource-demanding for networks in the near future. Using AI to select representative end users for generating digital twins and optimizing digital twin models may reduce the resource consumption of maintaining and updating digital twins. One potential implementation is using AI to categorize end users and select a portion of users from each category for creating digital twins. Alternatively, since it may be more challenging to provide QoE guarantee for some end users than others, using AI to select such end users for creating digital twins can potentially reduce the resource consumption on digital twins for 6G networks.               



\subsection{Potential Network Architecture for 6G: A Summary}
This section has provided a potential network architecture for 6G, which integrates two key  elements, i.e., pervasive network intelligence and holistic network virtualization. In the proposed network architecture, detailed network components, subsystems, and potential implementation have been discussed. Moreover, three types of interplay in the architecture are provided to characterize the proposed network architecture.

The proposed network architecture holds great potential for achieving advanced network management schemes and supporting AI services in 6G networks. Firstly, integrating  digital twins and network slicing facilitates user-centric networking and improves the granularity of network management. Secondly, integrating data-driven methods and model-driven methods enables novel hybrid data-model driven methods, which has the potential to outperform existing network management methods in terms of adaptivity, granularity, and so on. Thirdly, leveraging the network slicing concept in AI services facilitates AI services targeting QoS performance guarantees.




% Although data-driven methods, i.e., AI techniques, will play a critical role in network management by learning  directly from extensive raw data, they have several limitations, especially in non-stationary environments. First, data-driven methods are difficult to be generalized in new scenarios as they have strong dependency on data. If data-driven methods are applied in  scenarios that have never been experienced before, it is likely to observe severe performance deterioration due to a mismatch between the data the AI models were trained on and the data they encounter in new scenarios. Second, new scenarios may trigger the AI model retraining process. Model retraining from scratch requires collecting extensive data samples and waiting thousands of training epochs until satisfactory model accuracy is achieved, which results in prohibitive data collection cost and long training delay~\cite{yang2020deep}. %Hence, only relying on data-driven methods to manage the network maybe insufficient. % 加几个文献



%Model-driven methods can be a complement to data-driven methods, which often work in a ``model-then-optimize" manner. Mathematical models can be constructed to characterize the relations among key variables for a considered problem. Then, based on the constructed mathematical models, optimization schemes are developed. For instance, convex optimization algorithms can be applied if the considered problem is convex. Compared with data-driven methods, the model-driven methods have multiple advantages. First, the constructed models are general and can be used in a range of different network scenarios, including scenarios that are not known yet~\cite{zappone2019wireless}. {For instance, a channel fading model can be applied in various wireless networks by tuning model parameters.} Second,  once mathematical models are constructed, model-driven methods can be applied instantly, without a time-consuming model training process. % 加几个文献



% In 6G networks, the data-driven and model-driven methods should be applied in synergy for network management, resulting in \emph{hybrid data\&model driven methods}. Compared with the two individual methods, the hybrid methods can achieve the following advantages:

% \begin{itemize}
%     \item \emph{Mutual complement} - These two methods can complement each other to deal with network management problems under different scenarios: (1) The data-driven methods may focus on managing large-scale complex networks. Adopting model-driven methods to manage ultra-dense networks with a large number of end users is difficult due to a large number of variables and complicated relations among them. Moreover, the computational complexity of model-driven methods may increase exponentially with the number of variables and become prohibitive. In such case, data-driven methods can leverage DNNs to capture the implicit and complicated relation, yielding efficient and effective solutions; (2) The model-driven methods may focus on dealing with newly encountered situations. Unlike the data-driven methods that suffer from performance deterioration and long training delay in new situations, the model-driven methods with the constructed mathematical models can provide sub-optimal yet effective solutions in new situations;
%     \item \emph{Mutual enhancement} - These two methods can also enhance each other in multiple manners: (1) The data-driven methods can provide essential information for model-driven methods. For instance, DL-based traffic prediction can help model-driven resource management by providing traffic demand prediction; (2) The model-driven methods can generate data for the data-driven methods. For instance, a DNN model can be first trained on a large amount of synthetic data generated from a model-driven scheme, and then an extra training process based on real-world data can be applied to refine the DNN model~\cite{zappone2019wireless}. In this way, the cost of collecting real-world data can be significantly reduced; (3) The data-driven and model-driven methods can collaboratively make decisions for different sub-problems. For instance, data-driven methods may focus on tightly coupled decisions in large-scale networks  (e.g., resource reservation decisions among multiple BSs), and model-driven methods may focus on loosely coupled or independent decisions in small-scale networks (e.g., resource scheduling decisions at individual BSs)~\cite{J_WWu2020}. By properly decoupling the decision process, the hybrid  methods may find the optimal network management policy in complicated network scenarios.
% \end{itemize}
% %\begin{itemize}



%Therefore, these two methods can complement each other . %example











==> Final version/sec_acronyms.tex <==
~~~\,~~~
\begin{tabular}{ll}
5G  & Fifth Generation \tabularnewline

ABC & Always Best Connected \tabularnewline
AI & Artificial Intelligence \tabularnewline
AP & Access Point \tabularnewline
AR & Augmented Reality \tabularnewline

BBU & Base Band Unit  \tabularnewline
BRNN & Bidirectional Deep Recurrent Neural Network\tabularnewline
BS & Base Station \tabularnewline

CapEx & Capital Expenditure \tabularnewline
CNN & Convolution Neural Network \tabularnewline

D2D & Device-to-device  \tabularnewline
DNN & Deep Neural Network \tabularnewline
DCF & Distributed Coordination Function \tabularnewline
DSRC & Dedicated Short-range Communications \tabularnewline

eMBB & Enhanced Mobile Broadband \tabularnewline

FTP & File Transfer Protocol \tabularnewline

HARQ & Hybrid Automatic Repeat-request \tabularnewline
HNN & Hopfield Neural Network\tabularnewline

IoT & Internet of Things\tabularnewline

LFU & Least Frequently Used\tabularnewline
LRU & Least Recent Used\tabularnewline
LSTM & Long Short-Term Memory \tabularnewline
LTE & Long Term Evolution \tabularnewline

MDP & Markov Decision Process \tabularnewline
MEC & Mobile Edge Computing \tabularnewline
ML & Machine Learning \tabularnewline
mMTC & Massive Machine-type Communications \tabularnewline

NFV & Network Function Virtualization  \tabularnewline

OpEx & Operational Expenditure \tabularnewline

POMDP & Partially Observable Markov Decision Process \tabularnewline

QoS & Quality of Service \tabularnewline


\end{tabular}

~~~\,~~~
\begin{tabular}{ll}
RAN & Radio Access Network \tabularnewline
RAT & Radio Access Technology \tabularnewline
RL & Reinforcement Learning\tabularnewline
RNN & Recurrent Neural Network  \tabularnewline
RSU & Road-Side Unit \tabularnewline

SDN & Software Defined Networking\tabularnewline
SLA & Service Level Agreement \tabularnewline

UAV & Unmanned Aerial Vehicle \tabularnewline
URLLC & Ultra-reliable and Low-latency Communications \tabularnewline

V2X & Vehicle-to-everything \tabularnewline
VNF & Virtual Network Function \tabularnewline
VNO & Virtual Network Operator \tabularnewline
VR & Virtual Reality \tabularnewline







\end{tabular}

==> Final version/sec_conclusions.tex <==
Designing an architecture for future networks is challenging, especially when the use cases and defining techniques are still beneath the surface. Nevertheless, the evolution of networks through the previous generations demonstrates a necessity to support increasingly heterogeneous networks, diverse services, and stringent QoS/QoE requirements. This has been driving the trend of virtualization and generating significant interest in AI-driven networking. Recognizing the insufficiency of the existing scope and level of virtualization and AI for future 6G networks, we have presented a conceptual architecture design that integrates holistic network virtualization and pervasive network intelligence. To complement and solidify our overall network architecture, we have proposed several specific designs, including the six-layer holistic network virtualization based on digital twins, the connected AI solution for network management, as well as ideas, including AI slices and hybrid data-model driven methods. As a result, the proposed network architecture has the potential to achieve unprecedented scalability and flexibility due to the holistic network virtualization as well as exceeding adaptivity and intelligence due to the pervasive network intelligence. At last, we have identified some challenges and open issues related to the proposed architecture. We hope this study will lead to further discussions and developments on the architecture of 6G networks.

\section*{Acknowledgement}
The authors would like to thank Dr. Dongxiao Liu for helpful discussions on open issues related to data privacy and security.

==> Final version/sec_introduction.tex <==
\subsection{Background}

With the ongoing worldwide deployment of the 5th generation (5G) networks, the technical community in wireless communications and networking has started looking into the 6th generation (6G) networks for 2030 and beyond. While the exact concepts and techniques that define 6G are not determined yet, visions, requirements, use cases, and candidate techniques are discussed in an increasing amount of works, e.g., \cite{J_You2021towards, M_WSaad_2020, M_MGiordani_2020}. Among these  discussions, some preliminary consensus regarding 6G emerges. For instance, in terms of main requirements of 6G, the urgency of improving security~\cite{MNet_XShen_2020} and energy efficiency~\cite{J_ASodhro_2020} is understood unanimously. For use cases of 6G, the combination of enhanced mobile broadband (eMBB), ultra-reliable and low-latency communications (uRLLC), and massive machine-type communications (mMTC) have been brought up, despite the different terminologies used in different works \cite{M_ZZhang_2019}, \cite{M_BZong2019}. As to candidate techniques, commonly mentioned examples include the integration of satellite, aerial, terrestrial, and underwater networks~\cite{M_NZhang}, \cite{M_SChen_2020}, (sub)terahertz and visible light communications~\cite{M_ECStrinati2019}, artificial intelligence (AI) empowered networks~\cite{J_XShen_2020, M_KLetaief2019, yang2020artificial}, to name a few.              

One consensus deserving special attention is that 6G may need a brand-new network architecture. Driven by cost effectiveness and efficiency, the evolution of network architecture follows the evolving services provided by the networks. For instance, to introduce data service, a packet-switched core network component emerged in the 3G architecture as a complement to its circuit-switched counterpart for voice service~\cite{M_MSayed_2002}. Then, to accommodate the exponential growth of data traffic, 4G introduced a redesigned and simplified network architecture for a flat all-Internet protocol (IP) network with increased data rate and reduced latency~\cite{M_BBjerke_2011}. In the era of 5G, as networks become more heterogeneous than ever while services become diversified, various network architecture innovations have been proposed towards  flexible service-oriented networking, including software defined networking (SDN) \cite{S_DKreutz_2015}, cloud radio access network (C-RAN) \cite{S_AChecko_2015}, and network slicing~\cite{J_MBagaa2018}, \cite{J_WWu2020}. Therefore, envisioned to support unprecedentedly diverse services with exceedingly stringent quality of service (QoS) or quality of experience (QoE) requirements, 6G will most likely need ground-breaking innovations in network architecture.    

While conceiving an architecture for 6G, it is difficult to overlook two key elements, i.e., virtualization and AI. Network virtualization already plays an important role in the architecture of 5G~\cite{M_KQu_2020}. The virtualization of resources, functions, and networks enables resource sharing, software implementation of network functions, and service-orientated networking, respectively, and thereby increases resource utilization while reducing the cost for deploying and operating networks. Virtualization reflects a trend of softwarization for flexible, scalable, and adaptive network management~\cite{S_IAfolabi2018}. Therefore, it is foreseeable that virtualization will remain crucial in the architecture of 6G. As for the second key element, i.e., AI, a growing number of research teams worldwide are investigating AI-driven networks, and high expectation is placed on AI for empowering 6G~\cite{J_You2021towards, O_Ali6gWhite_2020}. In comparison with  heuristic or mathematical model based approaches for communications and networking, AI based approaches can handle complicated networking  problems and obtain accurate results, provided that sufficient data are available for training. This advantage suits the increasingly heterogeneous and dynamic networks, where mathematical models may not exist or cannot accurately characterize the considered problems. Therefore, it is not difficult to predict the significance of AI in 6G.         

\subsection{Architectural Innovations Required for 6G}

Recognizing the importance of virtualization and AI, we further look into their limitations in the state-of-the-art to comprehend the architectural innovations required for 6G. Existing virtualization techniques mostly deal with \textit{service provision} in communication networks. For instance, network slicing highlights available network resources, service provision capability, and QoS satisfaction for various services~\cite{J_HZhang2016}. While such virtualization, with a focus on service provision, enables 5G to handle diverse coexisting services, it may not suffice for 6G since the characteristics of end user \textit{service demand} can be the key to achieving user-centric networking. Therefore, in the future, virtualization should focus on both the service provision capability of a network and the service demand of end users in the network. This will lead to the virtualization of end users in addition to the virtualization of networks. As for AI, existing research on AI mostly addresses specific functions (e.g., routing~\cite{S_Fadlullah2017}),  layers (e.g., physical layer~\cite{J_AToma2020}), network segments (e.g., access networks~\cite{M_SHan2020}), or applications (e.g., autonomous driving~\cite{J_MLi2021}) of a network. Meanwhile, how to integrate AI into the network architecture across different layers or network segments needs further investigation. The scope and extent of AI-driven networks are yet to be determined.         

As virtualization extends to cover both service provision and service demand while AI pervades every corner of the network, close connections between the two elements are foreseeable and can dominate the architectural needs of 6G. The first connection is through network and end user \textit{data}~\cite{li2021slicing}. Virtualization facilitates the characterization of network service provision capability, service performance, resource utilization and, in future networks, end user service demand. As a result, a vast amount of data will be generated, which can be exploited to characterize the network and end users. Such data, if properly managed, can empower both AI-driven networking and AI applications (e.g., object detection)~\cite{O_PChemouil2020}. The second connection is through network \textit{control}. AI can be used to make decisions pertinent to virtualization, including service admission, slice establishment, dynamic virtual network function orchestration, and resource scheduling. In the future, AI can also help control data collection for the virtualization of end users and extract features of virtualized end users. Thus, AI has the potential to improve the efficacy and adaptivity of virtualization. The third connection is through network \textit{resources}. A main motivation of network virtualization is to coordinate resource sharing among different services and thereby improve network resource utilization and service satisfaction. AI-driven networking can target efficient utilization of network resources. As both virtualization and AI consume computing, communication, and storage resources, they may compete for network resources. However, AI has a potential to increase the efficiency of virtualization through intelligent network planning and operations, while virtualization may increase the efficiency of AI through proper data provision and management. As a result, they should work together to enhance network resource utilization and service quality.          

%For instance, a main motivation of virtualization is to coordinate resource sharing between different services and thereby improve resource utilization. Meanwhile, AI-driven networking will demand abundant computing (e.g., for training and inference), storage (e.g., for data management), and communication (e.g., for data collection or distributed training) resources. While AI consumes network resources, it could also support virtualization by improving resource management strategies.             

%The first connection is through \textit{resources}. For instance, existing virtualization techniques such as network function virtualization (NFV) rely on virtual machines and/or cloud computing and require abundant computing resource to operate \cite{S_VNguyen2017}. Undoubtedly, AI enabled network management would also demand abundant computing resource.

%Thus, to support virtualization and AI, the architecture of 6G must support flexible and efficient coordination of network resources.


%In future networks, when virtualization extends to the aspect of service demand, as aforementioned, and characterize the communication and networking demands of all users for all services, a vast amount of information about end users can be generated. Such information, if well-organized, can be used to feed and power AI for making predictions and decisions, such as network planning and scheduling, for network management.         


%Virtualization and AI are closely related, and it is necessary to understanding their connection while conceiving an architecture for 6G. In existing networks, virtualization enables flexible abstraction and allocation of computing, communication, and caching resources, which is the prerequisite for integrating AI into every corner of a network. In future networks, when virtualization extends to the aspect of service demand, as aforementioned, and characterize the communication and networking demands of all users for all services, a vast amount of information about end users can be generated. Such information, if well-organized, can be used to feed and power AI for making predictions and decisions, such as network planning and scheduling, for network management.         


A rudiment of the above connections through data and control can be observed in the existing architecture of 5G. For instance, the 3rd Generation Partnership Project (3GPP) introduces a network data analytics function (NWDAF) for 5G in Release 15~\cite{3gpp.29.520} and enablers for network automation (eNA) in Release 16~\cite{3gpp.21.916}. The architecture design provides a framework for the NWDAF to collect data from other network functions (such as policy control and network slice selection functions) and provide analytics (such as data traffic statistics and predictions) back to these network functions. In 6G, the scope and level of both data collection and analytics will expand significantly. Most likely, network data analysis, instead of being limited to one or two specific functions, will be AI-driven and available everywhere in a network. Similarly, the data available for network management, instead of being limited in type, content, or format, should provide information of the network and end users as needed. Such expectations can be fulfilled by extending the roles of virtualization and AI in the network architecture.  

\subsection{Our Vision}

Our vision of network architecture for 6G is based on the importance of virtualization and AI, their limitations in existing networks, and the essential connections between them. Specifically, we aim to design a network architecture that i) supports virtualization of the network and  end users from the perspectives of service provision and service demand, respectively, ii) integrates  AI  in various network functions, layers, segments, and applications under a unified architecture, and, more importantly, iii) facilitates the interplay between virtualization and AI, enabling their coexistence, integration, and mutual enhancement. To consolidate the vision, we raise the following three key questions: 
\begin{itemize}
	\item How to further advance virtualization beyond network slicing?    
	\item How to enable AI into every facet of a network?     
	\item How to effectively integrate virtualization and AI through network architecture design? 
\end{itemize}

In pursuit of answering the preceding questions, we develop the ideas of holistic network virtualization and pervasive network intelligence for 6G network architecture. \textit{Holistic network virtualization} advances virtualization toward 6G by incorporating network slicing and digital twin paradigms. The former enables service-centric network management, and the latter adds a user-centric perspective to virtualization for future networks. \textit{Pervasive network intelligence} enables generic integration of AI into a network from the perspectives of AI for networking and networking for AI. The former emphasizes the role of AI in network management, while the latter leverages network design to support AI applications. In this tutorial paper, for both holistic network virtualization and pervasive network intelligence, we survey existing studies, present our network architecture designs, and illustrate their benefits. Unifying these two components, we further introduce an overall conceptual network architecture, which fulfills our vision of unprecedentedly flexible, scalable, adaptive, and intelligent networks for 6G.           

 \begin{figure*}[tt]
	\centering
	\renewcommand{\figurename}{Fig.}
	\includegraphics[width=1\textwidth]{Fig/fig11.pdf}
	%	\vspace{0cm}
	\caption{The structure of this paper.}
	\label{fig:structure}
\end{figure*}


This tutorial paper can provide useful information and benefit readers from three aspects. First, for readers who are interested in the historical and current developments of virtualization and AI techniques, we survey the literature and provide a review of both in the context of communication networks. Second, for readers who are exploring future directions in virtualization and AI, we propose original ideas for advancing them toward 6G. Specifically, we illustrate designs and ideas, such as incorporating digital twins for holistic network virtualization, connected AI for network management, AI slices with training and inference separation, and hybrid data-model driven methods, throughout this paper. Last, after introducing our vision of holistic network virtualization and pervasive network intelligence, we present open issues and challenges to inspire further research.
%Readers of this tutorial paper can find useful informational from both the review of virtualization and AI techniques in existing networks and the original ideas that we propose for advancing them for 6G networks. Specifically, we illustrate designs and ideas such as incorporating end user digital twin for holistic network virtualization, connected AI for network management, AI slices with training and inference separation, hybrid data-Model driven method and so on throughout this paper. 


There are a few surveys on virtualization and AI in the literature~\cite{S_IAfolabi2018, J_RMinerva_ProcIEEE_2020,boutaba2018comprehensive, zhang2019deep}. Regarding virtualization, Minerva \emph{et al.} present existing digital twin based applications in the context of IoT~\cite{J_RMinerva_ProcIEEE_2020}, and another survey introduces the key enabling technologies and design principles of network slicing~\cite{S_IAfolabi2018}. Regarding AI, Boutaba \emph{et al.} undertake a comprehensive survey on AI applications in various areas of networking~\cite{boutaba2018comprehensive}, and another survey focuses on  deep learning (DL) based applications in wireless networking~\cite{zhang2019deep}. In comparison, this tutorial paper focuses on the vision of 6G. Specifically, after introducing state-of-the-art virtualization and AI techniques, we propose original designs, including holistic network virtualization and pervasive network intelligence, to establish a novel conceptual architecture for 6G networks. 



\subsection{Structure of the Paper}

  
The structure of this tutorial paper is shown in Fig.~\ref{fig:structure}.

Section~\ref{sec:HNV} illustrates our vision of 6G networks from the aspect of holistic network virtualization. We review existing network virtualization concepts and techniques in Subsection~\ref{ss:NetVirtual}. Then, we introduce end user virtualization with a focus on digital twins in Subsection~\ref{ss:EUVirtual}. Lastly, we present our idea of holistic network virtualization, highlighting a six-layer virtualization architecture, in Subsection~\ref{ss:HNV}. 


Section~\ref{sec:PI} illustrates our vision of 6G networks from the aspect of pervasive network intelligence. Subsection~\ref{ss:AIOv} presents an overview of representative AI techniques that are potentially useful for 6G networks. Subsection~\ref{ss:Moti} introduces the motivation for pervasive network intelligence and presents a four-level AI architecture. Subsections~\ref{ss:AIforNet} and \ref{ss:NetforAI} summarize the existing research and present our ideas on AI for networking and networking for AI, respectively.

Section~\ref{sec:PNA} integrates holistic network virtualization and pervasive network intelligence and presents our overall vision for 6G. Subsection~\ref{ss:related6Garc} reviews related studies on architectures for 6G. Subsection~\ref{ss:ArcOv} introduces a conceptual architecture for 6G networks that incorporates holistic network virtualization and pervasive network intelligence. Subsections~\ref{ss:comp}~and~\ref{ss:Implement} discuss the components, subsystems, and potential implementation of the proposed architecture. Subsections~\ref{ss:IntDTNS}~to~\ref{ss:IntVTAI} elaborate on three types of interplay enabled by the proposed architecture, i.e., the interplay between digital twin and network slicing, between data-driven and model-driven methods, and between virtualization and AI, respectively.

Section~\ref{sec:Open} identifies key challenges and open issues related to the proposed network architecture, and Section~\ref{sec:conclusions} concludes this research. 

Table~\ref{t:acronym} lists the acronyms used in this paper.

\begin{table}
\footnotesize 
% \normalsize
\centering
\captionsetup{justification=centering,singlelinecheck=false}
\caption{List of Acronyms}\label{t:acronym}
\begin{tabular}{l|l}
\hline\hline
3GPP & 3rd Generation Partnership Project \\
5G & 5th Generation \\
6G & 6th Generation \\
AI & Artificial Intelligence \\
AL & AI Level \\
AP & Access Point \\
API & Application Programming Interface \\
ARQ & Automatic Repeat-Request \\
BS & Base Station \\
C-RAN & Cloud Radio Access Network \\
DL & Deep Learning \\
DNN & Deep Neural Network \\
DRL & Deep Reinforcement Learning \\
eMBB & Enhanced Mobile Broadband \\
FL & Federated Learning \\
% eNA & Enablers for Network Automation \\
IoT & Internet of Things \\
IP & Internet Protocol \\
ITU & International Telecommunication Union \\
LSTM & Long Short-Term Memory \\
LTE & Long Term Evolution \\
mMTC & Massive Machine-Type Communications \\
MIMO & Multiple-Input Multiple-Output\\
ML & Machine Learning \\
NFV & Network Function Virtualization \\
NN & Neural Network \\
% NLP & Natural Language Processing \\
% NOP & Network Operation Policy \\
% NPP & Network Planning Policy \\
NWDAF & Network Data Analytics Function \\
QoE & Quality of Experience \\
QoS & Quality of Service \\
RAN & Radio Access Network \\
SBS & Small Base Station \\
SDN & Software Defined Networking \\
SNR & Signal-to-Noise Ratio \\
UAV & Unmanned Aerial Vehicle \\
uRLLC & Ultra-Reliable and Low-Latency Communications \\
VL & Virtualization Layer \\ 
VM & Virtual Machine \\
WSN & Wireless Sensor Network \\ 
\hline\hline
\end{tabular}
\end{table}

%The role of the second key factor, i.e., AI, in 6G network architecture can be understood from two aspects: AI-enabled network management and network-enabled AI services. The former emphasizes the role of AI in network data analysis, resource management, and service provision, while the latter leverages network design and networking techniques to support AI applications~\cite{O_PChemouil2020}. Accordingly, the architecture of 6G should exploit AI to facilitate the provision of conventional network services and, at the same time, support the emerging AI services~\cite{C_S_Parsaeefard2019}. 

% For example, virtualization in 5G focuses on the network side, i.e., network resources, status, and service provision capabilities, but not the end user side, i.e., service demand and user QoS/QoE.

%Both "pervasive"\\
%virtualization: node link resource network\\
%AI: device, edge, cloud\\

%data, flexibility\\
%control\\

%Virtualization and AI are closely related, and their first connection is \textit{computing}. Existing virtualization techniques such as network function virtualization (NFV) rely on virtual machines and/or cloud computing and require abundant computing resource to operate \cite{S_VNguyen2017}. Undoubtedly, AI enabled network management would also demand abundant computing resource. Thus, to support virtualization and AI, the architecture of 6G must support flexible and efficient coordination of computing resource in the network. The second connection between virtualization and AI is \textit{data}. The cyber space of any physical network, with virtual resources, functions, users, and networks therein, is essentially composed of a vast amount of data. Such data can provide information regarding the performance of virtual networks as well as the service demand of users. As a result, the following interplay may exist in the architecture of 6G: properly selected and organized data is provided by virtualization to power AI, while AI refines virtualization based on the provided data. Through the above loop, AI and virtualization enhance each other.              

%A rudiment of the above interplay can be observed in the existing architecture of 5G. For instance, 3GPP introduced a network data analytics function (NWDAF) for 5G in release 15~\cite{3gpp.29.520} and enablers for network automation (eNA) in release 16~\cite{3gpp.21.916}. Such architecture design provides a framework for collecting data from other network functions, such as policy control or network slice selection functions, and providing analytics, such as statistics and predictions, back to the network functions. In 6G, the scope and level of both data collection and analytics will witness significant progresses. Most likely, network data analysis, instead of being limited to one or two specific functions, will be AI-driven and available everywhere in the physical or cyber space of a network. Similarly, the data available for network management, instead of being limited in types, content, or formats, will be able to provide any information regarding any object in the physical or cyber space of a network as needed.  

    
%Achieving the above feature requires a brand new network architecture that enables the interplay (! not focus on this; 3 parallel) and mutual enhancement between virtualization and AI. The objective of this paper is to propose ideas for such architecture. To achieve this objective, we raise three key questions while investigating the architecture of 6G:
%\begin{itemize}
%	\item How to further advance virtualization?    
%	\item How to integrate AI-enabled network management and network-enabled AI services?    
%	\item How to facilitate the interplay between virtualization and AI through their connection in data and computing resource? 
%\end{itemize}
%In the pursuit of answers to the above questions, we develop the idea of holistic network virtualization and pervasive network intelligence based network architecture for 6G. Holistic network virtualization extends existing virtualization to cover the virtualization of end users and network slices with the introduction of two levels of digital twins. The architectural design of holistic network virtualization enables a flexible, adaptive, and customizable approach to organize the vast amount of data in the cyber space of a network. The approach enables a thorough characterization of service demands, network service provision capacity, resource utilization, user QoE/QoS, etc., supports the collection of selected and organized data for analysis and decision making, and allows changes to the content, format, accuracy, and update frequency of data based on the need of network management or services(!reduce!).  \textcolor{blue}{[add description and advantage of pervasive network intelligence architecture here]}         


%In the rest of the paper, we elaborate our idea for 6G network architecture, starting from holistic network virtualization. 


%will be virtualized, ubiquitous, and AI-driven. However, enabling the interplay between virtualization and AI in the network architecture of 6G .  
%
%
%Analytics functions will be virtualized, ubiquitous, and AI-driven, while data will play a vital role in network management. However,    
%
%data comprehensive functions will be AI-driven.
% 
%Despite the promising outlook, connecting virtualization and AI through data can be challenging. Unlike any other resource, data are a valuable resource but also consume network resources to transfer, store, and process. As the cyber space of a network has a vast amount of data, covering all services, network resources, and users, the cost may outweigh the benefit without a proper design to select and organize data for various AI functions and applications of the network. 
%
%
%A challenge for enabling the above loop in the architecture of 6G is 
%
%The two factors are closely related: computing, data.
%
%For data analysis, AI may empower functions in the 6G network architecture similar to the network data analytics function (NWDAF) introduced by 3GPP for 5G~\cite{3gpp.29.520}. 
%
%
%From the perspective of network management and service provision, various data are of interest. Examples include but are not limited to data describing the following: 1) On a large scale - spatial-temporal distribution of service-specific traffic volume, network configuration and resource allocation, network resource utilization, network-wide service level agreement satisfaction, etc. and 2) On a small scale - user location and mobility, content popularity, server computing load, user QoS/QoE, etc. The above data reflect service demand, network status, or service provision capacity and thus have great value for evaluating and refining network control and resource management. Recognizing the importance of data, 3GPP introduced enablers for network automation (eNA), an architecture enhancement of 5G and a framework for data collection to support data analytics in its Release 16~\cite{3gpp.21.916}. Nevertheless, major network architecture innovations, rather than enhancements, would be necessary to fully exploit the value of data in 6G. 
%
%
%Data may have a unique role in the architecture of 6G. Specifically, data are a resource, yet the transferring, storing, and processing of data consume network resources. 
% 
%The unique feature of data renders any   
%
%any network architecture design should unique characteristic of data    
%
%
% 
%
%data is a resource, using data consumes resource: properly chosen and organized data have more value.
%
%precondition for AI: cloud computing, cheap device, algorithm, data; AI facilitates service provision (previous work on AI-assisted slicing), AI is also a prevailing service (cite examples) to be supported by 6G.
%
%In the existing networks, data logger are used. not well organized.   
%
%
%
%
%AI 
%
%or example, for content delivery      
%
%next-generation network
%
%recent architecture innovations, cloud RAN, SDN
%
%future trends/requirements
%
%metric: security, energy efficiency
%components: SAG+ underwater; mmWave, (sub)terahertz, VLC; AI; new Architecture
%
%
%converged integrated network, access techniques, so on
%
%converged in the physical space (access, infrastructure), diverse in the cyber space (control, management)
%
%
%
%virtualization, slicing architecture
%
%AI, learning architecture
%


==> sec_acronyms.tex <==
~~~\,~~~
\begin{tabular}{ll}
5G  & Fifth Generation \tabularnewline

ABC & Always Best Connected \tabularnewline
AI & Artificial Intelligence \tabularnewline
AP & Access Point \tabularnewline
AR & Augmented Reality \tabularnewline

BBU & Base Band Unit  \tabularnewline
BRNN & Bidirectional Deep Recurrent Neural Network\tabularnewline
BS & Base Station \tabularnewline

CapEx & Capital Expenditure \tabularnewline
CNN & Convolution Neural Network \tabularnewline

D2D & Device-to-device  \tabularnewline
DNN & Deep Neural Network \tabularnewline
DCF & Distributed Coordination Function \tabularnewline
DSRC & Dedicated Short-range Communications \tabularnewline

eMBB & Enhanced Mobile Broadband \tabularnewline

FTP & File Transfer Protocol \tabularnewline

HARQ & Hybrid Automatic Repeat-request \tabularnewline
HNN & Hopfield Neural Network\tabularnewline

IoT & Internet of Things\tabularnewline

LFU & Least Frequently Used\tabularnewline
LRU & Least Recent Used\tabularnewline
LSTM & Long Short-Term Memory \tabularnewline
LTE & Long Term Evolution \tabularnewline

MDP & Markov Decision Process \tabularnewline
MEC & Mobile Edge Computing \tabularnewline
ML & Machine Learning \tabularnewline
mMTC & Massive Machine-type Communications \tabularnewline

NFV & Network Function Virtualization  \tabularnewline

OpEx & Operational Expenditure \tabularnewline

POMDP & Partially Observable Markov Decision Process \tabularnewline

QoS & Quality of Service \tabularnewline


\end{tabular}

~~~\,~~~
\begin{tabular}{ll}
RAN & Radio Access Network \tabularnewline
RAT & Radio Access Technology \tabularnewline
RL & Reinforcement Learning\tabularnewline
RNN & Recurrent Neural Network  \tabularnewline
RSU & Road-Side Unit \tabularnewline

SDN & Software Defined Networking\tabularnewline
SLA & Service Level Agreement \tabularnewline

UAV & Unmanned Aerial Vehicle \tabularnewline
URLLC & Ultra-reliable and Low-latency Communications \tabularnewline

V2X & Vehicle-to-everything \tabularnewline
VNF & Virtual Network Function \tabularnewline
VNO & Virtual Network Operator \tabularnewline
VR & Virtual Reality \tabularnewline







\end{tabular}
